Beyond the Phase Ordering Problem: Finding the Globally Optimal Code w.r.t. Optimization Phases

In this paper, we propose a new concept called \textit{semantically equivalence} \wrt \textit{optimization phases} \textit{(\sep)}, which defines the set of programs a compiler considers semantically equivalent to the input using a set of optimization phases. We show both theoretically and empirically that solving the phase ordering problem does not necessarily result in the most efficient code among all programs that a compiler deems semantically equivalent to the input, hereinafter referred to as the global optimal code \wrt optimization phases. To find the global optimal code \wrt optimization phases, we present a conceptual framework, leveraging the reverse of existing optimization phases. In theory, we prove that the framework is capable of finding the global optimal code for any program. We realize this framework into a technique, called \textit{iterative bi-directional optimization (\tool)}, which performs both the normal and reverse optimizations to increase and decrease the efficiency of the generated code, respectively. We evaluate \tool on C/C++ files randomly extracted from highly mature and influential programs (\eg, Linux kernel, OpenSSL, Z3). Results show that \tool frequently generates more efficient code -- measured by either code size or runtime performance -- than exhaustive search, which is the solution to the phase ordering problem. We also find by simply incorporating \tool's reverse optimization phases, the effectiveness of the optimization of state-of-the-art compilers (\eg, GCC/LLVM) can be significantly improved.

==> discussion.tex <==
\section{DISCUSSION}
In this section, we summarize the major lessons and takeaways that we have learned from conducting this work.

\subsection{Curbing False Positives}

False positives mainly arise from the imprecision of our performance estimation method in Algorithm~\ref{alg:cc}. In our evaluation, we find that the factor that accounts for most of the false positives (over 40\%) is the 
instruction-level parallelism which our cost model (adopted from LLVM) does not consider. Moreover, when our deoptimizations 
affect the cost model in projecting how loops are unrolled when estimating the performance of loop constructs, false positives also rise up (close to 40\%). While improving our cost model is a viable option, it is adopted from LLVM's cost model which represents the state-of-the-art, and improving LLVM's cost model requires significant domain knowledge which falls beyond the scope of this work. Therefore, we tackle the false positives issues in the following ways.


First, our static performance estimation method should prioritize code according to their size. That is, when code size is small, their instructions are less complex (\ie, without extensive instruction parallelism). As a result, our estimation is more precise. In fact, we find that when the reduced program produced by Algorithm~\ref{alg:cc} has less than 40 instructions, the false positive ratio is less than 20\%. Second, we should also rank the reduced program based on the savings in the cost of instructions generated from its deoptimized version (\ie, $cost(R_c) - cost(R_c')$ where $cost$ is our cost model). The higher the saving is, the higher the reduced program should be ranked. We find that when the saving normalized by the cost of instructions of the machine code generated from the reduced program is over 15\% (\ie, $(cost(R_c) - cost(R_c'))/cost(R_c) > 15\%$), the false positive ratio is less than 15\%.
Finally, even though dynamic profiling can be inaccurate in measuring block-level performance (as explained in Section~\ref{subsec:per}), exploring hardware-level profiling is a promising future direction due to its precision and efficiency. 


\subsection{Takeaway for Compiler Developers}

A clear implication of our research for compiler developers is that they can simply follow our methodology to uncover compiler defects previously unknown to them. Specifically, compiler developers can apply the deoptimizations proposed in this work to their seed programs for testing compilers, and run the compiler on both the original seed and deoptimized variant to generate the machine code. If the machine code generated from the deoptimized variant is more optimized than that generated from the original seed, this indicates a potential compiler defect that warrants further investigation.

Another important lesson that our findings provide to compiler developers is that when they design a new optimization or modify an existing one, the updated optimization should not suppress other optimizations which if applied could lead to more performant code generated. An experiment that compiler developers can design to validate compilers in light of updated optimizations is to first carefully create the test programs to which multiple chains of optimizations are applicable including both the existing and updated optimization. Then, compiler developers can perform a differential testing on the same test program using two versions of the compiler (\ie, before and after the change on optimizations). Finally, check the results of both runs, if the machine code generated by the old version of the compiler happens to be more performant than that generated by the new version, then it is a defect related to the updated optimization that compiler developers should look into.

\subsection{Helping Application Developers}

Given the presence of the compiler defects discovered in this work, our method provides a temporary workaround to application developers before these compiler defects get fixed. In particular, we can run our method to find the deoptimized version of their code for which compiler generates more optimized machine code. Developers can update their original code based on the deoptimized one to improve the performance of their applications. In fact, we have proposed \gfjc{5} patches for performance bugs that we identified with two of them already accepted by application developers.

==> eval.tex <==
\section{EVALUATION}
\label{sec:eva}

% \wyc{todo} 
% This section presents our evaluation. We start by introducing our experiment setup (Section~\ref{sec:eval:setup}). Then, we describe the results of our evaluation, and discuss a few examples of the compiler defects that we have found, resulted in the suboptimal code generated for the original programs (Section~\ref{sec:eval:reportedbugs}). Next, we show the diversity of discovered compiler defects, relating to a wide range of compiler components and real-world programs (Section~\ref{sec:eval:diversity}). Finally, we compare our approach against existing methods in finding missing compiler optimizations (Section~\ref{sec:eval:comparedce}). 

% guideline:

% since existing compilers focus on phase ordering, we investigate when we incorporate global ordering into compiler, examine the difference 

% \ke{TO do for yu}

% now introduce the setup, and other minor details (implementation, etc.)

% \ke{TO do for yu}

% we can say we will present the results in the subsection~\ref{}....7.1,2,3

% \subsection{RQ1}

% set up the background, fill in the blanks for numbers later.

% \subsection{RQ2}

% same here

% \subsection{RQ3}

% same here.

\wyc{TODO: 
discuss universal transformations.
}

Existing literature primarily addresses phase ordering problems in compiler optimizations. We introduce \prob, offering a novel approach to compiler optimizations. In our evaluation, we examine the differences between incorporating \prob into compiler optimizations and relying exclusively on the phase ordering problem. Specifically, we assess whether our approach can effectively enhance the efficiency of code generated by compilers.
\ke{should emphasize if incorporating our idea can indeed help compilers generate more efficient code in practice.}


\subsection{Experiment Setup}
We discuss in detail the whole evaluation procedure. First, we collect \ke{construct sounds like we are creating while we are only selecting...} programs from real-world projects to build an evaluation dataset. For each program in the dataset, we apply the phase ordering method and our method in turn to optimize each program, then we compare the results of both methods.


\noindent\textbf{\textit{Implementation.}}\, 
We implement our approach in a tool, \tool, in particular, we use LLVM's optimization to build universal transformations. 

\vspace{3pt}
\noindent\textbf{\textit{Test corpus.}}\, As phase ordering is time-consuming, we focus on function-level optimization in our experiment. The real-world functions are collected from \textit{AnghaBench}~\cite{anghabench} and \textit{llvm-opt-benchmark}~\cite{opt-benchmark}, which include 15 various open-source projects like \textit{Linux, QEMU, jemalloc, Redis, OpenSSL, NumPy, PHP, z3} \etc. Next, we randomly select functions across the selected projects. Finally, we build a dataset with a total of XXX functions. \ke{Yu, pls explain how do you select the 433 functions.}


\vspace{3pt}
\noindent\textbf{\textit{Phase Ordering Baselines.}}\, \wyc{To discuss: we need multiple baselines, at least one exhaustive and one sota.}
As shown in \textit{PhaseOrdering} function in Algorihtm~\ref{alg:cc}, we use a brute-force approach that exhaustively tries all combinations of optimizations. However, as the search space is very large, we can apply several strategies such as random search, depth-first search, breadth-first search, \etc 
In our experiment, we select the random search strategy due to its diversity, which allows us to explore a wide range of optimization sequences. In contrast, the other two strategies lack this advantage.
\ke{should mention we use a timeout, can not run forever for all programs...}
To reduce the time taken for the approach, we incorporate a simple, efficient but sound static analyzer~\cite{babati2017static} that identifies whether an optimization can be applied to a given program, according to the basic pattern of the optimization. For example, we will not try arithmetic optimization if a program does not have any arithmetic computations. 
% It is obvious that the static analyzer can only reduce the search space of phase ordering, to avoid solving the phase ordering problem endlessly, we assign 48 hour time budget for each run.
It is evident that the static analyzer can only reduce the search space of phase ordering. To prevent an endless search for a solution, we allocate a 48-hour time budget for each run.
\ke{very likely, reviewers going to ask you how does this static analysis work? is it sound? what kind of sensitivity?....hongyu, I would suggest that you provide the details you think are important and necessary in the process of implementing this. }
\chyc{We should design static analysis for specific types of optimization, such as natural loop recognition. For example, a program without loop cannot be optimized by loop-related optimization.}


\vspace{3pt}
\noindent\textbf{\textit{Setup of \prob.}}\, 
Similar to the running time budget for baselines, we also give \prob 48-hour time budget for each run.
% Note that in \prob, the number of universal transformations and optimizations applied also follows the threshold. 
\ke{hongyu, try giving more details about the implementation like above.} \chyc{todo}

\vspace{3pt}
\noindent\textbf{\textit{Hardware.}}\,
We run \tool on a 48-core Intel Xeon machine with Ubuntu 22.04 and 32GB memory.



The results are presented in the following subsections, each addressing a specific research question:
\begin{itemize}[leftmargin=*]
    % \item \textbf{\textit{RQ1}}:\, How difficult is it for us to find a better-optimized program than the best-optimized program found by phase ordering? 
	\item \textbf{\textit{RQ1}}:\, Can \prob more effectively find the global optimal program compared to \spo?
    \item \textbf{\textit{RQ2}}:\, Would we always find a more optimal program as the depth of universal transformations (\ie, $|s_1|$) increases? 
    \item \textbf{\textit{RQ3}}:\, What are the heuristics that guide the project developers in optimizing/deoptimizing their code to find more optimal programs to benefit developers? \wyc{1. what kinds of programs are better for our method? 2. how often can the heuristics be applied?}
\end{itemize}


\subsection{RQ1: Effectiveness in finding more optimal programs for our method than phase ordering}\label{sec:eval:effective}


This RQ is the basic evaluation of \prob, answering whether \prob is useful in real-world programs. 


\vspace{3pt}
\noindent\textbf{\textit{Setup of \prob.}}\, 
We employ random search to explore universal transformation sequences, as this experiment aims to evaluate the effectiveness of our method and phase ordering. Both breadth-first search and depth-first search may stuck in a narrow search space, thereby impeding the discovery of optimal programs. 

\vspace{3pt}
\noindent\textbf{\textit{Metric.}}\,
For a given program, we count the number of programs that our method can find a more optimal program than phase ordering. Then we divide the number by the total number of programs we have evaluated. 

\vspace{3pt}
\noindent\textbf{\textit{Results.}}\, 



\subsection{RQ2: Usefulness of increasing the depth of universal transformations}\label{sec:eval:useful}
In this RQ, we assess whether the global optimal programs become stable as the distance between the transformed program $s_1(P_o)$ and the original program $P_o$ increases. The answer can help us find an efficient heuristic to apply the universal transformations.

\vspace{3pt}
\noindent\textbf{\textit{Setup of \prob.}}\, 
This evaluation investigates whether an increased number of transformations contributes to the discovery of optimal programs. To this end, we employ a depth-first search to explore universal transformation sequences. Because depth-first search prioritizes applying the maximum number of transformations, aiding in identifying relationships between programs with fewer and those with more transformations applied.


\vspace{3pt}
\noindent\textbf{\textit{Metric.}}\,
As illustrated in Algorithm~\ref{alg:cc}, for a program $P_o$, the distance between $s_1(P_{o})$ and $P_{o}$ is given by $d=|s_1|$. We use $\mathcal{P}_d$ to denote the set of programs obtained by transforming $P_o$ through $d$ universal transformations. The frequency of discovering optimal programs at distance $d$ is calculated as the number of more optimal programs found by \prob divided by the total number of programs. Specifically,
\[ f_d = \frac{|\{P_o | P_o \in \mathcal{P}_d,  t(P_{o}')>t(\bar{P_o})\}|}{|\mathcal{P}_d|} \]
For each program in our dataset, we calculate $f_1, f_2, \dots, f_n$. We then average $f_i$ over all programs, where $i \in [1, 2, \dots, n]$.


\vspace{3pt}
\noindent\textbf{\textit{Results.}}\,

\subsection{RQ3: Heuristic Guidance for Project Developers} \label{sec:eval:guidedeveloper}
This research question helps us understand how the global optimal programs obtained from the transformed program $s_1(P_o)$ vary with different distances and types of universal transformations. These findings can guide developers in selecting appropriate universal transformations.

\vspace{3pt}
\noindent\textbf{\textit{Experiment Setup.}}\, 
Unlike the previous two experiments, we have designed a new experiment to answer this question.
The core idea of the experiment is to measure the contribution of each universal transformation in help phase ordering find the optimal programs.
In particular, we select XXX programs that our method finds more optimal programs. Then, for each program, we pick its corresponding universal transformation sequence. Finally, we incorporate the idea of Shapely Value\wyc{todo}~\cite{xxx} to measure the importance of each transformation in the transformation sequence. 

\vspace{3pt}
\noindent\textbf{\textit{Metric.}}\, 
The importance of a transformation is calculated by averaging the Shapely Value~\wyc{todo} of the transformation for each program.

% \vspace{3pt}
% \noindent\textbf{\textit{Setup of \prob.}}\, 
% This evaluation investigates how different transformations contribute to the discovery of optimal programs. Therefore, we use a breadth-first search to explore universal transformation sequences. \wyc{We set the length of universal transformation to be XXX according to the conclusion of RQ2.}

% \vspace{3pt}
% \noindent\textbf{\textit{Metric.}}\, 
% \wyc{to discuss: illustrate the results of one transformation is clear, how to present the results of two or more transformations.}
% We designed XXX transformations. We use $\mathcal{P}_t$ to denote a set of programs transformed from $P_o$ by transformation $t$.
% The frequency of discovering optimal programs by transformation $t$ is calculated as the number of more optimal programs found by \prob divided by the total number of programs.
% \[ f_t = \frac{|\{P_o | P_o \in \mathcal{P}_t,  t(P_{o}')>t(\bar{P_o})\}|}{|\mathcal{P}_t|} \]
% For each program in our dataset, we calculate $f_1, f_2, \dots, f_{XXX}$ \wyc{todo}. We then average $f_i$ over all programs, where $i \in [1, 2, \dots, XXX]$.



\noindent\rule{10cm}{0.4pt}



We implement our approach in a tool, \tool\wyc{todo}, in particular, we use LLVM's optimization to build universal transformations.

We aim to answer the following research questions regarding our proposed problem:

\begin{itemize}[leftmargin=*]
    % \item \textbf{\textit{RQ1}}:\, How difficult is it for us to find a better-optimized program than the best-optimized program found by phase ordering? 
	\item \textbf{\textit{RQ1}}:\, 
 
baseline
 
 %Is \prob easier to find the global optimal program than \spo? 
    Can \prob more effectively find the global optimal program compared to \spo?
    %\item \textbf{\textit{RQ2}}:\, What is the time taken to find the optimal program when the length of the universal transformation sequence (\ie, $|s_1|$) increases?
    \item \textbf{\textit{RQ2}}:\, Would we always reach a better optimal program as the depth of universal transformations increases? 
    \item \textbf{\textit{RQ3}}:\, What are the heuristics that guide the project developers in optimizing/deoptimizing their code to find more optimal programs to benefit developers? \wyc{1. what kinds of programs are better for our method? 2. how often can the heuristics be applied?}
    \item \textbf{\textit{RQ4}}:\, Can we find better-optimized programs compared to existing superoptimizers?
\end{itemize}


\textbf{RQ1} answers the frequency and time taken of \prob to find the global optimal program compared to \spo, as the distance $d$ ($d = |s_1|$) between the transformed program $s_1(P_o)$ and the original program $P_o$ increases.
For \textbf{RQ2}, we assess whether the global optimal programs become stable as the distance between the transformed program $s_1(P_o)$ and the original program $P_o$ increases.
\textbf{RQ3} shows whether the global optimal programs remain unchanged once the distance between the transformed program $s_1(P_o)$ and the original program $P_o$ reaches a certain threshold.
\textbf{RQ4} helps us understand how the global optimal programs obtained by the transformed program $s_1(P_o)$ vary as the distance and types of universal transformations vary. This finding could guide developers select universal transformations.
Finally, \textbf{RQ5} evaluates whether \prob could be an efficient alternative for superoptimizers.

% \gfjc{TODO Summary of Results?}



% \noindent\textbf{\textit{Methodology.}}\,
% To address \textbf{RQ1}, we evaluate the frequency and time taken of \prob to find the global optimal program compared to \spo, as the distance $d$ ($d = |s_1|$) between the transformed program $s_1(P_o)$ and the original program $P_o$ increases.
% For \textbf{RQ2}, we assess whether the global optimal programs become stable as the distance between the transformed program $s_1(P_o)$ and the original program $P_o$ increases.
% To answer \textbf{RQ3}, we evaluate whether the global optimal programs remain unchanged once the distance between the transformed program $s_1(P_o)$ and the original program $P_o$ reaches a certain threshold.
% To address \textbf{RQ4}, we examine the global optimal programs obtained by the transformed program $s_1(P_o)$ as the distance and types of universal transformations vary. 
% Finally, to answer \textbf{RQ5}, we compare the optimal program found in \textbf{RQ1} with Souper~\cite{sasnauskas2017souper}, a state-of-the-art and widely-used superoptimizer.


\subsection{RQ1: Effectiveness in finding the global optimal programs than phase ordering}\label{sec:eval:effective}

% \vspace{3pt}
\noindent\textbf{\textit{Experiment Setup.}}\,
% For a given input program $p_{k} (1\leq k\leq Total)$, we first use existing phase ordering tools\gfjc{TODO} to find its global optimal program $\bar{p_k}$. Then, we perform one universal transformation on $p_k$ to get $p_{k1}$, perform one universal transformation on $p_{k1}$ to get $p_{k2}$, and so on. The distance between $p_{ki}$ and $p_{k}$ is $i$. Next, we use the same phase ordering tool \gfjc{TODO} on $p_{ki}$ to find the optimized program $q_{ki}$. If $q_{ki}$ is more efficient than $\bar{p_k}$, \ie $Perf(q_{ki})>Perf(\bar{p_k})$, we say a better-optimized program than phase ordering's best-optimized program has been found.
% When the distance between the deoptimized program and the original program is $i$, the frequency of finding the better-optimized programs is $Count(Perf(q_{ki})>Perf(\bar{p_k}),1\leq k\leq Total)/Total$. 
For a given input program $P_{o} (1\leq o\leq Total)$, we first find its global optimal program $\bar{P_o}$. Then, we perform one universal transformation on $p_o$ to get $P_{o1}$, perform one universal transformation on $P_{o1}$ to get $P_{o2}$, and so on. The distance between $P_{oi}$ and $P_{o}$ is $i$. Next, we use the same phase ordering method on $P_{oi}$ to find the optimized program $P_{pi}'$. If $P_{oi}'$ is more efficient than $\bar{P_o}$, \ie $t(P_{oi}')>t(\bar{P_o})$, we say \prob can find the global optimal program while \spo cannot.
When the distance between the universal transformed program and the original program is $i$, the frequency of finding the global optimal programs is 
\[|\{P_o | P_o \in \mathcal{P}_i,  t(P_{oi}')>t(\bar{P_o})\}|/|\mathcal{P}_i|\] 

For each input program $P_{o} \in \mathcal{P}_i$, we also record the time taken to find the global optimal program by \prob and \spo. 
Finally, we define a cost $c$ as the number of transformations applied and require that both \prob and \spo should not apply more than $20$ transformations. \wyc{todo}

\vspace{3pt}
\noindent\textbf{\textit{Results.}}\, Table~\ref{table:eval:frequency} shows that the frequency of finding the better-optimized programs increases as the distance increases. This is because the farther the deoptimized programs are, the larger the search space.

Table~\ref{table:eval:time} shows that the time taken to find the better-optimized programs does not increase significantly as the distance increases.

The two tables show that not only we can find a more efficient optimized program than phase ordering, but also it won't take much time. Therefore, it is not hard to find a better-optimized program that is better than phase ordering's best solution.

\begin{table}
	\caption{The frequency of finding the better-optimized programs increases as the distance increases\gfjc{TODO line chart?}}
	\begin{tabular}{ |c | c | c | c|c|c|c|}
		\hline
		% Distance & Reported & Confirmed & Fixed \\
		% \hline
		Distance     & 0  & 1 & 2 & 3 & 4 & 5  \\\hline
		Frequency    &    &  &  &  &  &     \\
		\hline
	\end{tabular}
	\label{table:eval:frequency}
\end{table}

% \subsection{RQ2: The time taken to find the global optimal program when $|s_1|$ increases}\label{sec:eval:efficiency}

% \noindent\textbf{\textit{Experiment Setup.}}\, For each input program $p_{k} (1\leq k\leq Total)$, we also record the time taken to find the global optimal program than phase ordering's best-optimized program for each deoptimized program $p_{ki}$ (the distance from $p_{k}$ is $i (1\leq i\leq MaxDistance)$). 


% \vspace{3pt}
% \noindent\textbf{\textit{Results.}}\, Table~\ref{table:eval:time} shows that the time taken to find the better-optimized programs does not increase significantly as the distance increases.
% It shows that not only we can find a more efficient optimized program than phase ordering, but also it won't take much time. Therefore, it is not hard to find a better-optimized program that is better than phase ordering's best solution.


\begin{table}
	\caption{The time taken to find the better-optimized programs as the distance increases\gfjc{TODO}}
	\begin{tabular}{ |c | c | c | c|c|c|c|}
		\hline
		% Distance & Reported & Confirmed & Fixed \\
		% \hline
		Distance     & 0  & 1 & 2 & 3 & 4 & 5  \\\hline
		Time    &    &  &  &  &  &     \\
		\hline
	\end{tabular}
	\label{table:eval:time}
\end{table}


\subsection{RQ2: Usefulness of increasing the depth of universal transformations}\label{sec:eval:useful}

\noindent\textbf{\textit{Experiment Setup.}}\, We use the same setting as RQ1. However, in order to explore the relationship between the possibility of finding the global optimal and the sequence length of universal transformations, we need to increase the length of universal transformations. In this experiment, we set the maximum number of universal transformations to be $20$ and set the maximum number of optimizations to be $20$. 

\vspace{3pt}
\noindent\textbf{\textit{Results.}}\, 


\subsection{RQ3: Heuristic Guidance for Project Developers}\label{sec:eval:guidedeveloper}

\noindent\textbf{\textit{Experiment Setup.}}\, For each input program $P_{o} (1\leq o\leq Total)$, each time we perform one of the universal transformations on $P_{o}$ to get a transformed program $P_{oj}$. Finally, we get the optimized programs $P_{o1}'$, $P_{o2}'$, $\dots$, $P_{oj}'$. We will confirm which transformed program leads to less time in finding the global optimal program. In this setup, we set the maximum number of optimizations to be $20$. \wyc{incorrect}

\vspace{3pt}
\noindent\textbf{\textit{Results.}}\, 

\subsection{RQ4: Comparing with Existing Superoptimization Approaches}\label{sec:eval:comparesuper}

\noindent\textbf{\textit{Experiment Setup.}}\, We compare the optimal program found in \textbf{RQ1} with Souper~\cite{sasnauskas2017souper}, a state-of-the-art and widely-used superoptimizer.


\vspace{3pt}
\noindent\textbf{\textit{Results.}}\, 

==> evav2.tex <==
\section{Evaluation}
\label{sec:eva}

This section evaluates the effectiveness of \tool.
% As explained previously, from the theoretical perspective, compilers' omission of programs that are strictly less efficient than input programs during the optimization process cause them to generate suboptimal code. Now, we switch to the practical side, examining in real software development settings, how often existing compilers miss the global optimum for real-world code. 
In particular, we first describe in details our implementation of \FIBO{}.
% introduced in Section~\ref{subsec:real}, which is the cornerstone of this evaluation. 
Next, we present the results of our comprehensive evaluation of \tool, including a comparison with exhaustive search and state-of-the-art compilers --- GCC/LLVM. 

\subsection{The Implementation of Iterative Bi-Directional Optimizations}
We implement \FIBO{} within the LLVM infrastructure, which performs all transformations at the intermediate representation (IR) level --- transforming a given IR as input into a new IR as output. A key aspect of our implementation of \FIBO{} is selecting transformations to reverse. Since we have not solved the problem of identifying MOR, we 
% LLVM provides hundreds transformations, it would be highly challenging, if not unrealistic, to consider every one of them. To this end, we 
design the following criteria to guide our selection of transformations from the technical standpoint.

% \vspace{-4pt}
\begin{itemize}[leftmargin=*]
    \item \textit{\textbf{Influentiality:}} As we explained throughout the paper, the key objective of applying the reverse of transformations is to generate less efficient programs, which hopefully can be optimized into a more efficient version than the original program can be optimized into. This means that, at the very least, the less efficient programs must be optimized via a different sequence of optimizations than the original program. In this regard, we choose transformations that have a significant influence on others, meaning, reversing them would modify a wide range of code constructs, consequently, enable the application of many other optimizations. One particularly effective strategy we devise is to reverse an optimization $\alpha$, the result of which obstructs another optimizations $\beta$. Then, the third optimization $\gamma$ over which $\beta$ takes higher precedence can be applied, initiating a new sequence of optimizations that is not possible on the original program (as $\gamma$ cannot be applied due to the higher priority given to $\beta$). An illustrative example is the \textit{Mem2Reg} optimization in LLVM. This optimization identifies loads and stores of local variables, converting them into SSA-form. If \textit{Mem2Reg} is reversed, optimizations such as \textit{InstCombine} (an arithmetic optimization in LLVM), which feeds off the results of \textit{Mem2Reg}, can be obstructed. When \textit{InstCombine} is not applied, the information of range/bits will be preserved, which means optimizations like \textit{SCCP} (Sparse Conditional Constant Propagation), can leverage more precise range information for propagating integer constants.

    % \vspace{2pt}
    \item \textit{\textbf{Diversity:}} Another way to increase the chances of applying different optimization sequences to the less efficient programs is to make less efficient programs themselves more diverse. \textit{SimplifyCFG} optimization in LLVM is an example that serves the purpose. The optimization is responsible for merging basic blocks, collapsing redundant branches, and others to simplify Control-Flow Graph (CFG). Naturally, the reverse of \textit{SimplifyCFG} produces CFGs with a great deal of variety; furthermore, \textit{SimplifyCFG} can be repeatedly reversed to keep diversifying the less efficient programs. As a result, other optimizations related to CFGs such as \textit{JumpThreading} (which eliminates jumps between basic blocks) can be enabled.

    % \vspace{2pt}
    \item \textit{\textbf{Simplicity:}} We prioritize optimizations that are straightforward to reverse. Reversing LICM (loop invariant code motion) is a good example. We simply put an expression evaluated outside of the loop into the loop where the result of the evaluated expression is used. In contrast, we avoid optimizations that are difficult to reverse. Take dynamic loop unrolling (DCU) as an example. DCU partially unrolls a loop with a certain number of repetitions determined at run-time. This optimization can split a loop into multiple loops before the unrolling, making reversal highly complex. To reverse DCU, we need to perform sophisticated semantic analysis to determine precisely the potential influence that one separate loop has on the others and vice versa. Furthermore, unifying the bodies of the separate loops --- especially if they have diverged after the split --- into a single operation over the induction variable is also challenging. Most critically, we must ensure that the total number of loop iterations remains consistent after reversing DCU. Due to these complexities, we do not attempt to reverse such intricate optimizations as DCU.
          % unpredictable trip count, instead of repeating the body of a loop with trip count known at compile time. Dynamic Loop Unrolling inserts some preconditions and some payload before the unrolled loop to make unrolling legal. Thus, reversely, rerolling such a loop requires analyzing the semantics of its precondition and payload with the help of existing compiler analysis such as \textit{SCEV} (Scalar Evolution). It's nearly as difficult to implement rerolling as implementing unrolling. To avoid unnecessary workload, we tend to reverse optimizations satisfying the Simplicity standard .\ke{TODO: pls give a few very complicated optimizations that are difficult to reverse} \chyc{done.}
          % Meanwhile, real-world programs always show arithmetic optimization opportunities, a concrete example is that human tends to write down \texttt{a * 4} instead of \texttt{a << 2}. Reversing simple optimizations really empowers the impact compared to reversing other complex and uncommon optimizations.
\end{itemize}

According to the three criteria above, Table~\ref{table:transforms} lists all the transformations we choose to reverse. These optimizations target a broad range of code constructs, such as CFG, memory operations, and arithmetic expressions, ensuring the effectiveness of our implementation of \FIBO{} in handing a wide variety of programs.
With the set of transformations selected for reversal, we implement \FIBO{} according to Algorithm~\ref{alg:go}, which takes a program, the number of iterations $k$ as input and produces an optimized program as output.
% into a new optimization procedure, called \tool (\underline{O}ptimizations with \underline{R}everse \underline{T}ransformations). \ken{hongyu, you may give some details to make your implementation sounds well-versed}







\begin{table*}
    \captionsetup{skip=2pt}
    \caption{A list of reversed transformations.}
    \label{table:list}
    \centering
    \adjustbox{max width=1\textwidth}{
        \begin{tabular}{ | c | c | c|}
            \hline
            Optimization                                                                  & Description                       & Example of a reversal \\
            \hline
            \textit{InstCombine}                                                          & \tabincell{c}{Make instructions                           \\ more complex}&

            \begin{minipage}[m]{0.5\textwidth}
                \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
                \lstinputlisting[]{./code/mutation/instexpand.c}
            \end{minipage}
            \\
            \hline
            \textit{SimplifyCFG}                                                          & \tabincell{c}{Make control-flow                           \\more complex}  &
            \begin{minipage}[m]{0.5\textwidth}

                \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
                \lstinputlisting[]{./code/mutation/cfgexpand.c}

            \end{minipage}
            \\
            \hline
            \textit{Reassociation}                                                        & \tabincell{c}{Reassociate expres-                         \\sions in a non-canoni- \\ calized order} &
            \begin{minipage}[m]{0.5\textwidth}

                \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
                \lstinputlisting[]{./code/mutation/reassociate.c}

            \end{minipage}
            \\
            \hline

            \tabincell{c}{\textit{LICM}                                                                                                               \\ (Loop Invariant \\ Code Motion)}               &  \tabincell{c}{Put loop-invariants\\ into loops}&    \begin{minipage}[m]{0.5\textwidth}

                \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
                \lstinputlisting[]{./code/mutation/loopsink.c}

            \end{minipage}
            \\
            \hline

            \tabincell{c}{\textit{Mem2Reg}                                                                                                            \\ (Promote memory\\ to register)}                      & \tabincell{c}{Demote register\\ to stack}&
            \begin{minipage}[m]{0.5\textwidth}

                \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
                \lstinputlisting[]{./code/mutation/reg2mem.c}
                % \hline
            \end{minipage}
            \\
            % \hline
            % \tabincell{c}{ \textit{DCE}                                                                                                            \\ (Dead Code \\Elimination)}                       & \tabincell{c}{Randomly insert\\ dead code}  &
            % \begin{minipage}[m]{0.5\textwidth}

            %     \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
            %     \lstinputlisting[]{./code/mutation/dead.c}

            % \end{minipage}
            % \\
            \hline
            \textit{Loop Vectorizer}                                                      & \tabincell{c}{Scalarize the SIMD
            \\(Single Instruction/\\Multiple Data) \\ operations}  & \begin{minipage}[m]{0.5\textwidth}

                \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
                \lstinputlisting[]{./code/mutation/scalarize.c}

            \end{minipage}
            \\
            \hline

            \begin{tabular}{@{}c@{}}\textit{DSE}\,(Dead Store\\ Elimination)\end{tabular} & \tabincell{c}{Insert dead store                           \\ and move stores\\ around}                &
            \begin{minipage}[m]{0.5\textwidth}

                \lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none, basicstyle=\small\ttfamily\bfseries}
                \lstinputlisting[]{./code/mutation/clobber.c}

            \end{minipage}
            \\
            \hline
        \end{tabular}}
    \label{table:transforms}
    \vspace{-8pt}
\end{table*}

\subsection{Experiments}
\subsubsection{Comparing \tool with Exhaustive Search}\label{subsubsec:dir}
While Theorem~\ref{theo:subopt} reveals the issue with solving the phase ordering problem in theory, it remains to be seen if \tool can actually generate more efficient code than the solution to the phase ordering problem --- exhaustive search --- in practice. We aim to find out the answer in this evaluation. 

\tool, which is realized within the LLVM infrastructure, also performs exhaustive search as part of its workflow. Therefore, for consistency and easy integration, we implement exhaustive search using LLVM (the latest release at the time of this evaluation, \ie, LLVM 19.1.2). Since LLVM allows users to specify the ordering of optimization passes for a particular compilation through command lines, we provide all possible sequences of optimization passes enumerated in depth-first order as command line arguments. Each sequence of optimization passes saturates at the program to which no optimization passes can be applied,
% \footnote{LLVM limits the number for applying optimizations that can be applied indefinitely to prevent the code from growing too large}, 
\ie, the program is the result of applying that sequence of optimization passes to the input. 

\vspace{3pt}
\noindent\textbf{\textit{Test Programs.}}\,
We source test programs from two existing benchmarks: \textit{AnghaBench}~\cite{anghabench} and \textit{llvm-opt-benchmark}~\cite{opt-benchmark}. The former consists of the LLVM test suite (275 programs) 
and SPEC CPU\textsuperscript{\textregistered} 2006 (13 programs). 
The latter is an LLVM dataset for compiler optimization research, containing popular programs, such as Linux, QEMU, OpenSSL. Ensuring the significance of our evaluation, we focus on 15 well-established, highly influential programs, all of which have 10K+ stars on their Github repository. To reduce the complexity of test programs, we do not feed compilers a whole program. Instead, we use individual files of these 15 programs, which form the basic compilation unit. Considering that exhaustive search is an exponential-time algorithm, we randomly pick 50 files of single function, each with no more than 100 lines of code, on which the exhaustive search is feasible to run. We believe these files should provide sufficient data points for this evaluation without significantly prolonging our experiments. As previously explained, we consider all optimization passes in the LLVM -O3 pipeline to implement exhaustive search. However, since we target single function files, we filter out inter-procedural optimizations like IPSCCP (Inter-Procedural Sparse Conditional Constant Propagation) and function inlining.

% In particular, we randomly pick 217 C/C++ files from highly influential (with over 10K stars on their Github repository), real-world programs from these two benchmarks. Given the number of files used in this experiment, we should be able to draw a sound conclusion from our evaluation results. We leave compilers to process all inter-procedure calls within the same file as normal, and replace external function calls as global functions without bodies to make the file compile.x

\vspace{3pt}
\noindent\textbf{\textit{Machines.}}\,
We use three machines (of x86 architectures) throughout all of our evaluations:
Intel\textsuperscript{®} Core™ i7-12700H, Intel\textsuperscript{®} Xeon\textsuperscript{®} Platinum 9242, and AMD Ryzen™ 9 7950X, each of which has 32GB memory and runs Ubuntu 22.04.2 LTS.

\vspace{3pt}
\noindent\textbf{\textit{Process and Metrics for Evaluating the Code Efficiency.}}\,
A critical step in this experiment is to determine for the same file whether the code generated by \tool is more efficient than that generated by exhaustive search. More importantly, we investigate what contributed to the improved efficiency of the code generated by \tool if it is more efficient.

First, we pinpoint the part of an original C/C++ file which \tool and exhaustive search optimize into different IR respectively. In particular, we develop a reduction technique, which systematically removes other parts of the original file that do not lead to discrepancies in the IR generated by \tool and exhaustive search. A criterion we design to guide the reduction procedure is that the contrast between the IRs generated by \tool and exhaustive search must remain consistent before and after the reduction. For example, if the IR generated by \tool contains 5 fewer (or more) \myinline{add} instructions than that generated by exhaustive search for an original file, then the IR generated by exhaustive search must also contain 5 fewer (or more) \myinline{add} instructions for the reduced file. We utilize the automatic test case reducer~\cite{regehr2012test} to repeatedly remove some code at a time, until no more code can be removed without violating the above-mentioned criterion. To ensure the validity of reduced programs, we use CompCert's interpreter~\cite{compcertUB} to detect and eliminate undefined behavior if they appear.

Next, given the reduced file produced at the end of the previous step, we compile it into IR with \tool and exhaustive search. 


We assess the efficiency of generated code based on two well-established metrics — code size and runtime performance. To measure code size, we count the number of instructions in the IR generated by \tool and exhaustive search, respectively. If the IR produced by~\tool consists of fewer instructions, we then proceed to compare the runtime of each generated IR; otherwise, we terminate this process and mark the code generated by~\tool to be less efficient.



To measure the actual runtime of the generated code, we first use \myinline{llc} to compile LLVM IR generated by \tool and exhaustive search into assembly code towards each x86 architecture mentioned above. Regarding inputs for running the generated code, one way is to use test suites provided with each selected program. However, we find that executions under these inputs do not yield a sufficient coverage of the assembly code. On average, less than 50\% of the basic blocks are covered across all assembly code generated by either \tool or exhaustive search for each file. Therefore, we leverage AFL++~\cite{2020AFL} (with QEMU mode) to find inputs which should attain higher coverage than the provided test suites. 

For the assembly code produced by \tool and the exhaustive search for each C/C++ file on each architecture, we run AFL++ to find a common set of inputs that attain the full coverage of basic blocks in both assembly code. Next, we execute both assembly code generated for each file on each x86 architecture using the corresponding set of inputs discovered by AFL++, and record their running time. We consider the code produced by \tool for one file to be more efficient only if both the average and median running time of the code produced by \tool are shorter across all inputs on every architecture.

\begin{table}[t]
    \centering
    \captionsetup{skip=1pt}
    \caption{Comparing \tool with Exhaustive Search}
    \label{table:exhau}
    \begin{tabular}{|l|c|}
        \hline
        \diagbox{\tool}{Baseline} & Exhaustive Search      \\
        \hline
        % $k = 1$          & (7, 43)        \\
        % \hline
        % $k = 2$          & (14, 36)         \\
        % \hline
        % $k = 3$          & (20, 30)   \\
        % \hline
        % $k = 4$          & (21, 29)   \\
        % \hline
        % $k = 5$          & (22, 28)   \\
        % \hline\hline
        $k = 1$       & (13, 37)        \\
        \hline
        $k = 2$     & (20, 30)         \\
        \hline
        
    \end{tabular}
\end{table}

\vspace{3pt}
\noindent\textbf{\textit{Results.}}\,
The last two rows in Table~\ref{table:exhau} show the result of \tool and the exhaustive search. Since \tool performs iterations of bi-directional optimizations, the search space for the global optimum grows dramatically as the number of iterations $k$ increases. This is because the number of programs generated grows exponentially with the number of steps of reverse optimizations, in addition, the number of programs a generated program can be optimized into also grows exponentially in the exhaustive search. Given the computational resources at our disposal, we can only run \tool with $k \le 2$. When $k=2$, \tool generates more efficient code than exhaustive search for 20 out of 50 files. This result shows the frequency in which exhaustive search can miss the globally optimal code in practice. On the other hand, it also demonstrates the significant potential of our conceptual framework for finding the globally optimal code, considering that \tool is in fact a rather basic realization. Future, more effective instantiations, especially those can identify the MOR, should perform even better than exhaustive search.

\vspace{3pt}
\noindent\textbf{\textit{Examples.}}\, Figure~\ref{fig:ofslen} depicts a function for which \tool produced more efficient code than exhaustive search. The original function is extracted from QEMU, a widely used machine and userspace emulator and virtualizer. For brevity and clarity, we only show its reduced version (Figure~\ref{fig:oriex}).

For this function, the optimization that should have been performed is eliminating the body of the \myinline{if} clause from line 7 to 9 in Figure~\ref{fig:oriex}. Since the \myinline{if} condition at line 4 is equivalent to that at line 7, when the execution ever gets into the body of the \myinline{else} clause from line 7 to 11, the \myinline{if} condition at line 7 is guaranteed to be \myinline{false}. 

Exhaustive search did not find an ordering of LLVM's optimization passes that performs this optimization because it cannot find an ordering to derive the equivalence between the two \myinline{if} conditions. 
A natural question that may arise: why LLVM does not have an optimization pass that can switch side for \myinline{len} in either \myinline{if} condition, which would have made the equivalence between the two \myinline{if} conditions obvious. The reason is, switching sides for \myinline{len} does not make the resultant code more efficient, therefore, would not be performed by any optimization pass. For example, the \myinline{if} condition at line 7 \myinline{32 - len == ofs} takes one instruction of subtraction and another of equivalence check. If we move \myinline{-len} from left to right, the generated code \myinline{32 == ofs + len} still takes one instruction for addition and another for equivalence check. Given that addition and subtraction instructions run equally fast on modern x86 architectures, the transformation proposed above will not be performed.

\begin{figure*}[t]
    \captionsetup{skip=5pt}
    \centering
    \begin{subfigure}{0.32\linewidth}
        \captionsetup{skip=1pt}
        \raggedright
        \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\footnotesize\ttfamily\bfseries}
        \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example3-seed.c}
        \caption{}
        \label{fig:oriex}
    \end{subfigure}
    \;
    \begin{subfigure}{0.32\linewidth}
        \captionsetup{skip=1pt}
        \centering
        \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\footnotesize\ttfamily\bfseries}
        \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example3-mutant.c}
        \caption{}
        \label{fig:rev}
    \end{subfigure}
    \;
    \begin{subfigure}{0.32\linewidth}
        \captionsetup{skip=1pt}
        \raggedleft
        \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\footnotesize\ttfamily\bfseries}
        \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example3-mutantcompiled.c}
        \caption{}
        \label{fig:opt}
    \end{subfigure}

    \caption{(\subref{fig:oriex}) depicts the original function; (\subref{fig:rev}), which is resulted from the reverse optimizations, can be optimized into a more efficient code (depicted in (\subref{fig:opt})) than (\subref{fig:oriex}) can ever be optimized into (which is itself).}
    \label{fig:ofslen}
    \vspace{-10pt}
\end{figure*}

Figure~\ref{fig:rev} shows the program \tool generated by applying the reverse of \textit{InstCombine} in Table~\ref{table:list} to the original function. Notably, exhaustive search within \tool finds an ordering of optimization passes for this function that removes the redundant \myinline{if} clause mentioned earlier. Specifically, (1) it first switches \myinline{-32} in the \myinline{if} condition \myinline{(ofs + len) - 32 == 0} (line 4) from left to right, because doing so would eliminate the instruction for subtracting \myinline{32}, and the resultant code takes one instruction for adding \myinline{ofs + len} and another for comparing \myinline{ofs + len} with \myinline{32}. Next, (2) it transforms \myinline{(-len + 32) + (-ofs) == 0} (line 7 to 8) into \myinline{32 == (len + ofs)} through the following sub-steps: reassociating \myinline{(-len) + (-ofs)} to \myinline{-(len + ofs)} so that the minus sign can be applied once to the result of \myinline{(len + ofs)} instead of twice to \myinline{len} and \myinline{ofs} separately; and moving the entire expression \myinline{-(len + ofs)} across to the other side, which completely eliminates the minus sign, and generates \myinline{32 == (len + ofs)}. Finally, (3) it removes the dead \myinline{if} clause given that it recognizes the equivalence between \myinline{(ofs + len) == 32} and \myinline{32 == (ofs + len)}, resulted from the previous step. The optimized code is shown in Figure~\ref{fig:opt}. For interested readers, we have left a few more examples to the supplemental material.

% , whereas, the original code takes one instruction for the same addition operation and another for comparing \myinline{ofs + len} against \myinline{0}, in addition to the instruction for subtraction. 
% Similarly, for \myinline{((-len + 32) + (-ofs) == 0)} at line 7 to 8, exhaustive search finds an ordering of LLVM's optimization passes that does the following: (1) reassociating \myinline{(-len) + (-ofs)} to \myinline{-(len + ofs)} so that the minus sign can be applied once to the result of \myinline{(len + ofs)} instead of twice to \myinline{len} and \myinline{ofs} separately; (2) moving the entire expression \myinline{-(len + ofs)} across to the other side, which completely eliminates the minus sign, and generates \myinline{32 == (len + ofs)}. At this point, GCC/LLVM recognizes the two \myinline{if} conditions are equivalent, and subsequently removes the \myinline{if} clause that is deadcode. The optimized code is shown in Figure~\ref{fig:opt}. For interested readers, we have left a few more examples to the supplemental material.

\subsubsection{Improving the Optimization of State-of-The-Art Compilers}\label{subsubsec:dir}

Since there does not exist an efficient algorithm for solving the phase ordering problem, state-of-the-art compilers, such as GCC and LLVM, employ their own optimization pipelines. Therefore, a natural and relevant question is can we utilize our conceptual framework to improve the effectiveness of GCC/LLVM's optimizations? To answer this question, we adapt \tool for this evaluation. In particular, we replace exhaustive search in Algorithm~\ref{alg:go} with GCC/LLVM's optimization scheme, while keeping the rest of the algorithm intact. We then compare the efficiency of the code generated by \tool and GCC/LLVM directly. If \tool generates more efficient code, we conclude \tool can be utilized to improve the optimization of GCC/LLVM. 

For both compilers, we use their latest release (14.2 for GCC and 19.1.2 for LLVM) at the time of this evaluation. We run -O3 optimization level for both GCC and LLVM, as it is the most aggressive optimization mode and likely to generate the most efficient code. Based on the adaption of \tool introduced above, we compare \tool against GCC and LLVM separately. When comparing \tool against a specific compiler, we configure \tool to run that compiler's -O3 optimization (\eg, \tool runs LLVM's -O3 when compared against LLVM). Running LLVM at -O3 within \tool is straightforward because \tool is implemented within the LLVM infrastructure. We simply run the \myinline{opt} tool at -O3 to optimize the IR that \tool produces after applying the reverse transformations. Integrating GCC into \tool is slightly more involved. We first convert the IR that \tool produces (with the reverse optimizations) into C files using \myinline{LLVM-CBE}. Then, we compile these files using GCC (at -O3) to generate the assembly code, which will be compared with the assembly code directly generated by GCC at -O3. 

We randomly pick 200 C/C++ files from the same set of programs used in the previous experiment, which should allow us to draw a sound conclusion from our evaluation results. In this experiment, we lift the restriction to single-function files, which is no longer necessary. We evaluate the efficiency of the code produced by \tool and GCC/LLVM as follows. First, we measure code size by counting the number of instructions in the generated code. In particular, when comparing \tool against LLVM, we count the number of instructions in the IR generated by each method respectively. When comparing against GCC, we count the number of instructions in the assembly code generated by GCC and \tool (following the methodology described earlier) for each hardware architecture. 
% If \tool produces fewer instructions in the assembly code for every architecture, we proceed to estimate their runtime performance; otherwise, we consider the code produced by \tool less efficient.
Then, we adopt the procedure described in the previous experiment for measuring the running time of code generated by \tool for a selected C/C++ file. For code generated by GCC/LLVM, we run the executable that they compiled from the entire program, and record the runtime for the selected files. Finally, we performed the same validation process to manually confirm whether the code generated by \tool is indeed more efficient. 



% Unlike the previous experiment, we do not proceed straight to the stage of fuzzing generated code to measure their runtime performance. Because the generated code in this experiment exhibits notably higher complexity, which makes it significantly more challenging for AFL++ to find inputs that achieve sufficient coverage. To address this issue, we design a reduction technique aiming to simplifying the original C/C++ files for further validation. The goal of this reduction step is to pinpoint the part of the generated code that is fully responsible for the potentially better optimizations that \tool performs compared to GCC/LLVM. To achieve this goal, we design the following criterion:
% % remove the part of the original program that does not contribute to the differences in the compiled code generated by \tool and a baseline. The criterion we design is that 
% the contrast between the code produced by \tool and that produced by a baseline must remain consistent before and after the reduction. For example, if the code produced by \tool contains 5 fewer (or more) \myinline{add} instructions than that produced by a baseline for the original program, then the code produced by \tool must also contain 5 fewer (or more) \myinline{add} instructions for the reduced program. We utilize the automatic test case reducer~\cite{regehr2012test} to repeatedly remove some code at a time, until no more code can be removed without violating the above-mentioned criterion. To ensure the validity of reduced programs, we use CompCert's interpreter~\cite{compcertUB} to detect and eliminate undefined behavior if they appear.

% Given the program produced at the end of the reduction step, we compile it into assembly code for each of the three hardware architectures. While GCC and \tool do this automatically, we use \myinline{llc} to compile LLVM IR into assembly towards all x86 architectures when comparing \tool with LLVM. Finally, we utilize AFL++ to find inputs which we use to execute the assembly code and measure their runtime, like we did in the previous experiment.






% To estimate the expected runtime, we utilize LLVM's cost model\footnote{\url{https://llvm.org/doxygen/CostModel_8cpp_source.html}},
% % ~\cite{llvmcostmodel}, 
% which assigns a cost to each instruction based on their expected execution time. For straight-line code, we sum the costs of all instructions as provided by LLVM's cost model. To account for branches, we calculate the cost of instructions in each possible branch. We then compute the average of these costs, assuming that each branch is equally likely to be executed. To deal with loops, we set the loop count to 100, \ie, multiplying the cost of instructions in the loop body by 100 to determine the total cost of a loop.
% While our procedure may not be the most precise for estimating performance of compiled code, it is fair: all compiled code whether they are produced by \tool or baselines are handled in the same way. When comparing \tool with LLVM and AutoPhase, we simply compute the total cost of instructions in the IR they generate. Only if the IR generated by \tool incurs a smaller total cost than that of LLVM and AutoPhase, we move onto the next phase of this evaluation process. For the comparison against GCC, we compute the total cost of instructions in all three assembly code generated by \tool and GCC for the three hardware architectures. More importantly, we require that instructions in every assembly generated by \tool consistently incur a smaller total cost than those generated by GCC. If this condition is met, the evaluation process continues; otherwise, the code generated by \tool is considered less efficient.

% The second phase is to reduce the corresponding source files for further validation, considering that original files can be quite large (up to hundreds of lines of code). 

% The central goal of this reduction step is to remove the part of the original program that does not contribute to the differences in the compiled code generated by \tool and a baseline. The criterion we design is that the contrast between the code produced by \tool and that produced by a baseline must remain consistent before and after the reduction. For example, if the code produced by \tool contains 5 fewer (or more) \myinline{add} instructions than that produced by a baseline for the original program, then the code produced by \tool must also contain 5 fewer (or more) \myinline{add} instructions for the reduced program. We utilize the automatic test case reducer~\cite{regehr2012test} to repeatedly remove some code at a time, until no more code can be removed without violating the above-mentioned criterion.
% To ensure the validity of reduced programs,
% % are It is also important to guard against the undefined behavior which may appear in reduced programs. 
% we use CompCert's interpreter~\cite{compcertUB} to detect and eliminate undefined behavior if they appear.
% % , ensuring that reduced programs are valid.

% Given the program produced at the end of the reduction step, we compile it into assembly
% code for each of the three hardware architectures. While GCC and \tool do this automatically, we use \myinline{llc} to compile LLVM IR into assembly towards all x86 architectures when comparing \tool with LLVM or AutoPhase. In the final phase of this evaluation process, we leverage AFL++~\cite{2020AFL} (with QEMU mode) to find a common set of inputs that achieves the full basic block coverage for both the assembly produced by \tool and the baseline for each hardware architecture. We then execute the assembly code generated by \tool and the baseline on each architecture using the corresponding set of inputs discovered by AFL++, and record the execution time for each input. We consider the code produced by \tool to be more efficient than that produced by the baseline only if both the average and median running time of the assembly produced by \tool are shorter across all inputs on every hardware architecture.
% . Second, we execute the assembly produced by \tool and the baseline with this set of inputs on the three x86 architectures introduced previously (Intel\textsuperscript{®} Core™ i7-12700H, Intel\textsuperscript{®} Xeon\textsuperscript{®} Platinum 9242, and AMD Ryzen™ 9 7950X), and record the time the assemblies take to run for each input on every hardware architecture. 
% We count the assembly produced by \tool to be more efficient than that produced by the baseline only if both the average and median running time of the assembly produced by \tool on all inputs is shorter on every hardware architecture. 

% and present them to LLVM developers for manual validation. \ke{what did they do, why they would do it...}We count the code produced by \tool to be most efficient only if we received confirmations from LLVM developers. \ken{The same procedure will be repeated for the comparison between \tool and each baseline. The results are presented in Table~\ref{table:eee}. As shown from the table}

\begin{table}[t]
    \centering
    \captionsetup{skip=1pt}
    \caption{Results of the comparison between \tool and each baseline. The first element of the tuple in each cell denotes \#files for which \tool produces \textit{strictly} more efficient code. The second number denotes the number of the remaining files.}
    \label{table:eee}
    \begin{tabular}{|l|c|c|c|}
        \hline
        \diagbox{\tool}{Baselines} & GCC       & LLVM       & AutoPhase \\
        \hline
        $k = 1$          & (40, 177) & (49, 168)  &  (207, 10)         \\
        \hline
        $k = 2$          & (99, 118) & (96, 121)  &  (210, 7)         \\
        \hline
        $k = 3$          & (114, 103) & (109, 108) & (212, 5)   \\
        \hline
        $k = 4$          & (119, 98) & (114, 103) &  (214, 3)   \\
        \hline
        $k = 5$          & (121, 96) & (116, 101) &  (214, 3)    \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \captionsetup{skip=1pt}
    \caption{Comparing \tool with LLVM -O3}
    \label{table:stats_exhau}
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        \multirow{2}{*}{\tool} & 
        \multicolumn{4}{c|}{LLVM -O3}
        \\ 
        \cline{2-5}
        & avg(ct) (s) & median(ct) (s) & avg(\#inst) & median(\#inst) \\
        \hline
        $k = 1$         & (0.66, 0.08) &  (0.59, 0.09) & (29.77, 28.96) & (21,18)       \\
        \hline
        $k = 2$          & (3.05, 0.08) & (2.73, 0.09) & (28.35, 28.96) & (21,18)         \\
        \hline
        $k = 3$          & (31.48, 0.08) & (29.68, 0.09) & (28.11, 28.96) & (19,18)    \\
        \hline
        $k = 4$          & (213.95, 0.08)  & (193.34, 0.09) & (28.06, 28.96) & (18,18)    \\
        \hline
        $k = 5$          & (1002.71, 0.08) & (927.22, 0.09) & (27.98, 28.96) & (18,18)    \\
        \hline
    \end{tabular}
\end{table}

\vspace{3pt}
\noindent\textbf{\textit{Results.}}\,
Table~\ref{table:eee} presents the results of \tool compared to all baselines. In each cell, the first value of the tuple represents the number of files for which \tool generates \textit{strictly} more efficient code at an iteration $k$ (specified by the row) than a baseline (specified by the column). Given that \tool is built upon the baseline it is compared to, we only count it to be successful if generates a different code that is more efficient than the code generated by the baseline. The second value is the number of the remaining files.
% \ken{Hongyu, pls continue from here for the new version} 
% \chyc{Below is true if we drop 100 additional virtual test cases in all baselines} 
As the table shows, the number of programs for which \tool produces more efficient code than a baseline increases as the value of $k$ increases. By the time $k = 3$, \tool already produces more code with higher efficiency than every baseline. The margin continues to widen with further increases in $k$. Considering that source code files used in this experiment are randomly picked from mature, real programs, this result indicates that state-of-the-art compilers like GCC/LLVM frequently fail to generate the global optimal code when compiling programs in the real-world (\ie, more than half of the time). Moreover, the reverse transformations \tool performs are crucial in generating the global optimal code. Finally, we find that AutoPhase is the least effective baseline in this experiment. However, this should be an expected outcome because the merging machine learning based techniques are not yet as powerful as the well-established compilers developed through decades of extensive research and development.

\subsubsection{The Comparison between \tool and Exhaustive Search} In this experiment, we compare \tool against exhaustive search, which can be deemed the solution to the phase ordering problem. If \tool prevails, it becomes crystal clear that solving the phase ordering problem is not equivalent to generating the globally optimal code. We choose to implement the exhaustive search using LLVM framework, which
requires far less efforts, compared to using GCC (in which case, we need to work with GCC's source code). With LLVM, we simply specify the ordering of the optimizations passes via a command line, instructing LLVM to optimize an input program.
% Furthermore, if \tool outperforms the exhaustive search implemented on top of all LLVM's optimization passes, our point is proven, given that both \tool and exhaustive search relies on the same set of optimization passes in LLVM. 
Specifically,%Regarding the implementation details of the exhaustive search, 
we enumerate all possible sequences of optimization passes in depth-first order. Each sequence of optimization passes saturates at the program for which no optimization passes can be applied. This means that the program is the result of that sequence of optimization passes.

Given that the exhaustive search is more powerful than LLVM, \tool cannot generate more efficient code than the exhaustive search for the programs where it did not generate more efficient code than LLVM in the previous experiment. For this reason, we sample randomly a subset of files used in the previous experiment where \tool generated more efficient code than LLVM. Moreover, since the exhaustive search is an exponential-time algorithm, we randomly pick 50 files of single function, each with no more than 100 lines of code, on which the exhaustive search is feasible to run. These files should provide sufficient data points for this evaluation, and at the same time keep our experiment from running too long. On these source code files, the exhaustive search takes on average a few hours per file to complete, with the longest taking under two days. We consider all optimization passes in the LLVM -O3 pipeline, but since we are targeting single function files, we filter out inter-procedural optimizations like IPSCCP (Inter-Procedural Sparse Conditional Constant Propagation) and Function Inlining.

We opt for a simpler procedure to evaluate the efficiency of the code produced by~\tool and the exhaustive search. The reason is that the number of code produced by the exhaustive search for one program can be very large, ranging from a few hundreds to hundreds of thousands. This makes the evaluation procedure designed for the previous experiment prohibitively expensive to run, especially since reducing the original program while maintaining the contrast among such a vast number of variants is almost infeasible. Instead, we mainly rely on the last step of the previous evaluation process, which is to directly measure the runtime of the assembly code when executed on inputs discovered by AFL++. Specifically, we first compile the IR produced by \tool and the exhaustive search for the three hardware architectures. Notably, if the total number of instructions in the code produced by \tool for every architecture is not consistently smaller, we consider the code to be less efficient. Otherwise, for the assembly code produced by \tool and the exhaustive search for each architecture, we run AFL++ to find common inputs that attain the full coverage of basic blocks in both assembly code. Given the smaller size of the program used in this experiment, running AFL++ proves to be efficient. The whole process takes under a week to complete. Finally, we execute both assembly code generated for each x86 architecture on the corresponding set of inputs discovered by AFL++, and record their running time. We consider the code produced by \tool to be more efficient only if both the average and median running time of the code produced by \tool are shorter across all inputs for every architecture.

\begin{table}[t]
    \centering
    \captionsetup{skip=1pt}
    \caption{Comparing \tool (w/wo Exhaustive Search) with Exhaustive Search}
    \label{table:exhau}
    \begin{tabular}{|l|c|}
        \hline
        \diagbox[width=14em]{\tool}{Results}{Baseline} & Exhaustive Search      \\
        \hline
        $k = 1$          & (7, 43)        \\
        \hline
        $k = 2$          & (14, 36)         \\
        \hline
        $k = 3$          & (20, 30)   \\
        \hline
        $k = 4$          & (21, 29)   \\
        \hline
        $k = 5$          & (22, 28)   \\
        \hline\hline
        $k = 1$ (with Exhaustive Search)        & (13, 37)        \\
        \hline
        $k = 2$ (with Exhaustive Search)        & (20, 30)         \\
        \hline
        
    \end{tabular}
\end{table}

The first five rows in Table~\ref{table:exhau} show the results of \tool compared to the exhaustive search. Again, we observe the number of programs for which \tool produces more efficient code increases as $k$ rises. In particular, when $k=3$, \tool outperforms the exhaustive search on 20 out of 50 files. This number keeps increasing, albeit slowly, as $k$ continues to grow. These results prove that even if the phase ordering problem is solved, applying the solution to an input program may still fail to generate the global optimal code.

\begin{table}[t]
    \centering
    \captionsetup{skip=1pt}
    \caption{Comparing \tool (w/wo Exhaustive Search) with Exhaustive Search}
    \label{table:stats_exhau}
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        \multirow{2}{*}{IBO} & 
        \multicolumn{4}{c|}{Exhaustive Search}
        \\ 
        \cline{2-5}
        & avg(ct) (s) & median(ct) (s) & avg(\#inst) & median(\#inst) \\
        \hline
        $k = 1$         & (0.38, 212.23) &  (0.37, 124.91) & (22.43, 20.59) & (14,13)       \\
        \hline
        $k = 2$          & (2.33, 212.23) & (2.26, 124.91) & (20.92, 20.59) & (13,13)         \\
        \hline
        $k = 3$          & (19.08, 212.23) & (16.16, 124.91) & (20.63, 20.59) & (13,13)    \\
        \hline
        $k = 4$          & (159.00, 212.23)  & (154.15, 124.91) & (20.53, 20.59) & (13,13)    \\
        \hline
        $k = 5$          & (898.72, 212.23) & (880.2, 124.91) & (20.41, 20.59) & (13,13)    \\
        \hline\hline
        $k = 1$ (with Exhaustive Search)        & (679.14, 212.23) & (630.21, 124.91) & (21.02, 20.59) & (12,13)       \\
        \hline
        $k = 2$ (with Exhaustive Search)        & (4895.23, 212.23) & (4521.33, 124.91) & (20.88, 20.59) & (11.5,13)        \\
        \hline
    \end{tabular}
\end{table}

\subsubsection{The Comparison between \tool (with Exhaustive Search) and Exhaustive Search} The previous experiment conducts an unfair comparison, considering that \tool still relies on LLVM for generating the most efficient code that LLVM is capable of. Whereas, the exhaustive search finds the truly optimal phase ordering for input programs. Therefore, we configure \tool to run the exhaustive search in this experiment, while the rest of experiment setup remains unchanged.

% In this experiment, we set \tool to perform exhaustive search for finding the optimal sequence of optimizations, instead of -O3, the original module built into \tool. Ideally, we expect \tool to generate more efficient programs than exhaustive search for even more input programs.

% \vspace{3pt}
% \noindent\textbf{\textit{Results.}}\,
The last two rows in Table~\ref{table:exhau} show the result of \tool (with exhaustive search) and the exhaustive search. Since \tool performs iterations of bi-directional optimizations, the search space for the global optimum grows dramatically as the number of iterations $k$ increases. This is because the number of programs generated grows exponentially with the number of steps of reverse optimizations, in addition, the number of programs a generated program can be optimized into also grows exponentially in the exhaustive search. Given the computational resources at our disposal, we can only run \tool with $k \le 2$. In fact, when $k=2$, \tool achieves the same result as it previously attained with $k=3$ without the exhaustive search. This confirms the potential utility of reverse optimizations, especially under the assistance of the exhaustive search.
% The efficiency of programs produced by \tool under $k = 1$ is greater than that under $k = 2$.

% \vspace{3pt}
% \noindent\textbf{\textit{Examples.}}\,
% \ken{Hongyu, same thing.}
% Figure~\ref{fig:example5} is code reduced from \textit{OpenSSL}. After applying the reverse of \textit{SimplifyCFG, InstCombine, Mem2Reg}, \myinline{src} is deoptimized into \myinline{mutant}, which has an impact on the process of the loop unrolling, CFG modification in compiler optimizations, and further affect how the compiler optimization makes use of bits information from the context.
% \\
% Figure~\ref{fig:example6} is code reduced from \textit{QEMU}.  After applying the reverse of \textit{SimplifyCFG}, \myinline{src} is deoptimized into \myinline{mutant}. The deoptimization affects how instructions are combined.

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.505\linewidth}
%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example5-mutant.c}
%         \end{subfigure}

%         \vspace*{-4pt}
%         \quad\quad\quad\quad \quad\quad\quad\quad \quad\quad\quad\quad $\boldsymbol{\downarrow}$ \textit{\texttt{compiled to}} \\
%         \vspace*{-4pt}

%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example5-mutantcompiled.c}

%         \end{subfigure}
%         % \vspace*{2pt}	
%         \caption{}
%         \label{fig:moti:ori}
%     \end{subfigure}
%     \vspace*{-5pt}
%     \,
%     \begin{subfigure}{0.475\linewidth}
%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example5-seed.c}
%         \end{subfigure}

%         \vspace*{-4pt}
%         \quad\quad\quad\quad \quad\quad\quad\quad \quad\quad\quad\quad $\boldsymbol{\downarrow}$ \textit{\texttt{compiled to}} \\
%         \vspace*{-4pt}

%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             % \lstinputlisting[morekeywords={Object, String, bool}]{./code/example1.c}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example5-seedcompiled.c}
%         \end{subfigure}

%         \caption{}
%         \label{fig:example5:mut}
%     \end{subfigure}
%     \vspace*{-5pt}
%     \caption{balabala}
%     \vspace{-4pt}
%     \label{fig:example5}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.505\linewidth}
%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example6-mutant.c}
%         \end{subfigure}

%         \vspace*{-4pt}
%         \quad\quad\quad\quad \quad\quad\quad\quad \quad\quad\quad\quad $\boldsymbol{\downarrow}$ \textit{\texttt{compiled to}} \\
%         \vspace*{-4pt}

%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example6-mutantcompiled.c}

%         \end{subfigure}
%         % \vspace*{2pt}	
%         \caption{}
%         \label{fig:moti:ori}
%     \end{subfigure}
%     \vspace*{-5pt}
%     \,
%     \begin{subfigure}{0.475\linewidth}
%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example6-seed.c}
%         \end{subfigure}

%         \vspace*{-4pt}
%         \quad\quad\quad\quad \quad\quad\quad\quad \quad\quad\quad\quad $\boldsymbol{\downarrow}$ \textit{\texttt{compiled to}} \\
%         \vspace*{-4pt}

%         \begin{subfigure}{\linewidth}
%             \lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=single,framexleftmargin=1.5em,basicstyle=\small\ttfamily\bfseries}
%             % \lstinputlisting[morekeywords={Object, String, bool}]{./code/example1.c}
%             \lstinputlisting[morekeywords={Object, String, bool},basewidth=0.52em]{./code/new-example/example6-seedcompiled.c}
%         \end{subfigure}

%         \caption{}
%         \label{fig:example6:mut}
%     \end{subfigure}
%     \vspace*{-5pt}
%     \caption{balabala}
%     \vspace{-4pt}
%     \label{fig:example6}
% \end{figure*}

% \subsection{Discussions}

% \ken{for hongyu:}
% 1. summarize how the value of $k$ affects the results in general (this means you can try generalizing the results from each experiment) \\
% The more $k$, the more efficient programs \tool produces. However, the more $k$, the weaker the improvement by \tool becomes.\\

% 2. find out what are the most popular transformations whose reverse lead to efficient code, you can even rank them.\\
% The reverse of \textit{InstCombine} and \textit{SimplifyCFG} are the most popular transformations whose reverse leads to efficient code. A possible cause is that real-world programs could always be applied with the reverse of them, and they do the most basic optimizations, which would fundamentally affect other optimizations. Accordingly, the reverse of them affects other optimizations as well.\\

% 3. what are some rules you can summarize from your results that help people discover the right transformation to reverse if they want an algorithm for the global optimum?\\
% \chyc{Simply improve $k$???}
% One possible principle is that if a specific optimization is available frequently in your program, apply the reverse of it frequently too. For programs with complicated control flow, apply the reverse of \textit{SimplifyCFG} more. For arithmetic-intensive programs, apply the reverse of \textit{InstCombine} more.

% 4. any weaknesses that prevent \tool from finding even more efficient code. This is a good place to talk about this.
% \begin{enumerate}
%     \item Lacks various deoptimizations
%     \item Massively increases compilation time.
%     \item Theoretically, the set of programs \tool could reach when optimizing program $P$ is a subset of all equivalent programs of $P$. That is, \tool can only get the global optimal of a subset of all equivalent programs of $P$.
% \end{enumerate}

% \subsection{Implications for Compiler Developers}

% Apart from real optimizations (transformations that improve program performance), it's always useful to design transformations that transform programs into a form that is easier for optimizations to analyze. Compiler developers always take the intuition that more optimized programs would further enable more optimizations, but that's not true. Deoptimizations serve as the accelerant for other optimizations as well. One important reason is that deoptimized programs may reveal the information that simpler programs cannot provide. For example, \myinline{a ^ b} is equivalent to \myinline{(a | b) - (a & b)}, but neither GCC nor LLVM supports precise range analysis on exclusive or given the range of operands. Instead, these compilers can fetch precise range information from bitwise or, bitwise and, and subtraction. For this reason, the counter-intuitive fact is that they get precise information from complicated expression \myinline{(a | b) - (a & b)} instead of simpler \myinline{a ^ b}, and optimize the former better at the stage of constant propagation. \\
% Meanwhile, the compilers lack canonicalization on many simple primitives. That is, even a fragment of some common and simple code is presented in many non-orthogonal forms. These primitives keep many different variants throughout the whole process of optimization, which requires generalizing the identical optimization for these variants of equivalent semantics. And compiler developers always miss such generalizations. A concrete example is the \myinline{select} intrinsics in LLVM, which is used to choose one value based on a condition, without IR-level branching\cite{llvm-select}.
% \myinline{select cond, A, B} is equivalent to \myinline{if (cond) A else B}, where \myinline{A} and \myinline{B} are pure values. The former is a single instruction, while the latter consists of multiple basic blocks and multiple instructions. They often co-exist in the procedure of optimization. However, in many cases, the reasoning component of the compiler optimization could resolve the latter, and ignore the former. When it comes to simplifying the constraints between conditions, the latter is often optimized better. For this reason, the expansion of \myinline{select} by the reverse of \textit{SimplifyCFG} enables better optimization in many cases. A lesson to be taken is that canonicalizing programs make a difference, which not only avoids the burden of implementing multiple similar optimizations for multiple different equivalent patterns but also improves the effect of optimization since no one can catch every corner case. Compared with checking every corner case, canonicalizing corner cases into normal cases is a better choice.
% \\
% \textbf{\textit{Application Developer,}}  Compiler is a very complex software working around the combination of numerous rules, algorithms, and passes. A tiny modification may lead to a completely different result. A concrete lesson we learned is, that never do premature optimization on simple things, such as replacing \myinline{a * 2} with \myinline{a << 1}. Firstly, compilers always perform such simple folds, a manual fold won't help. Meanwhile, it's impossible for you to control the effect of your simple manual modification after compiler optimization. When optimizing a real-world program, the interactions between different rules, algorithms, and passes cannot be simply predicted without insight into the source of the compiler. If you desire to improve the performance of your application. Instead of imitating some simple compiler optimization, you'd better provide the information that the compiler can't reason from the program. For example, tell the compiler that one of the function arguments is assumed to be restricted to a specific range. Anyway, stop manually performing simple optimizations that compilers have done. Keeping a deoptimized source may lead to a refined result.

% \begin{table}[t]
%     \captionsetup{skip=2pt}
%     \caption{Comparison between \tool (with Exhaustive Search) and Exhaustive Search}
%     \label{table:experiment3}
%     \centering
%     % k = 1
%     \begin{subtable}[t]{0.495\linewidth}
%         \begin{tabular}{ | c| c| }
%             \hline
%             Methods                 & \begin{tabular}{c}\#Compiled code is \\ the most efficient\end{tabular} \\
%             \hline
%             Exhaustive Search       & 37                                                                      \\
%             \hline\hline
%             \textbf{\tool($k$ = 1)} & \textbf{13}                                                             \\
%             \hline
%         \end{tabular}
%     \end{subtable}
%     % k = 2
%     \begin{subtable}[t]{0.495\linewidth}
%         \begin{tabular}{ | c| c| }
%             \hline
%             Methods                 & \begin{tabular}{c}\#Compiled code is \\ the most efficient\end{tabular} \\
%             \hline
%             Exhaustive Search       & 30                                                                      \\
%             \hline\hline
%             \textbf{\tool($k$ = 2)} & \textbf{20}                                                             \\
%             \hline
%         \end{tabular}
%     \end{subtable}
% \end{table}

==> expdesign.tex <==
\section{Experiment Design}

In this section, we present how to effectively find possible global optimal programs in our experiment. 

\subsection{High-level Workflow}
Figure~\ref{fig:workflow} depicts the high-level workflow of our experimental design. Given a program \po{}, we first design universal transformations (\ie, $\mathcal{D}$ in Definition~\ref{def:prob}) and use them to transform \po{} into new programs \pd{}. Then, we apply existing phase ordering methods to \pd{}. In the performance estimation phase, we estimate the performance of \pd{}. When $t(\pd) \geq T$ ($T$ is an anticaped execution time defined in Definition~\ref{def:prob}), we go back to \pd{} and do the phase ordering again. This procedure will continue until the performance is better than the original program or it reaches a threshold.
Finally, we compile the program and produce the optimal code. 
It is worth noting that the backward step relies on the phase ordering method we choose. An exhaustive search solution for phase ordering will guarantee the production of optimal programs with sufficient performance gain, so the backward step is unnecessary. However, machine learning-based methods~\cite{ashouri2017micomp, xx, xx} require the step because they cannot guarantee this property.

We discuss the major components below:
\begin{itemize}[leftmargin=*]
	% \item \textbf{\textit{Original Programs.}}\, Existing studies often opt for programs generated by random code generators (\eg, CSmith~\cite{yang2011finding}) to identify optimization bugs in compilers. However, in this work, we focus on real-world programs, which helps translate our findings to practice more seamlessly. 
	\item \textbf{\textit{Universal Transformation.}}\, The universal transformation transforms an original program \po{} to transformed programs \pd{} by the transformation set $\mathcal{D}$ (Definition~\ref{def:prob}). The transformation set consists of a sequence of transformations, including deoptimizations and performance-irrelevant transformations. Deoptimizations are constructed by inverting existing compiler optimizations. In order to apply transformation in $\mathcal{D}$, we design several strategies: \wyc{todo}, all of which are discussed in the next section.
	\item \textbf{\textit{Phase Ordering.}}\, We use the existing phase ordering tool \gfjc{TODO} to generate the best-optimized program for each transformed program. 
	% \item \textbf{\textit{Performance Checking.}}\, \wyc{maybe use runtime profilers?} Our performance checking encompasses two aspects: code size and expected runtime. We employ static performance checkers to evaluate whether the performance of the optimized program \pdc is less than $T$. If such a situation is observed, we conclude that an optimal program has been found.
\end{itemize}



\begin{figure}[t]
	\centering
	\includegraphics[width=0.7\linewidth]{pics/workflow.pdf}
	\caption{Overview of our approach.}
	\label{fig:workflow}
\end{figure}

\subsection{Universal Transformation}
% As explained in Section~\ref{sec:form}, there are potentially two approaches to generating programs with varying levels of efficiency. Considering our research is centered on real-world programs and compilers, which typically offer limited scope for optimization, we choose to perform universal transformations on an original program to produce more variants. 

Universal transformations consist of deoptimizations and optimization-irrelevant transformations.
We first discuss how to design deoptimizations and optimization-irrelevant transformations, and then illustrate how we apply universal transformations.
% We first introduce basic definitions for deoptimization, then discuss how to design deoptimizations, and finally, we give an algorithm for illustrating how to apply deoptimizations.




% To mutate a given seed program $P$ to $P'$, we design a bunch of semantic-preserving transformations. And assemble them randomly into a pipeline as a mutator.

\subsubsection{Designing Deoptimizations}
\wyc{8.27: simplicity, popularity (commonly used and impactful optimization), sustainability. give examples for each principle.}

To construct deoptimizations, we start by selecting a compiler optimization. Although any optimization can be chosen theoretically, we adopt two selection criteria in practice. We analyze interdependencies in the optimization pipeline and choose the top-N optimizations with the most significant influence on others~\cite{alfred2007compilers}. This approach helps us to filter out less important optimizations that are irrelevant to prominent analyses in the optimization pipeline (\eg, data flow, control flow analysis, or arithmetic operations). For example, \textit{data layout} optimization~\cite{prashantha2014implementing}, which moves a rarely accessed variable out of frequently accessed data structure, is not selected according to our criterion. Because such transformations do not affect data flow or control flow of programs. 
The second principle we adopt is that optimizations should be common and widely applied. This ensures that our focus is on common and widely applied optimizations and their corresponding deoptimizations, making our method applicable to other compilers. 

After selecting an optimization \opt, the next step is to invert \opt to construct a deoptimization \deopt. To perform this inversion, we introduce a simple model of compiler optimizations. We consider an optimization \opt as consisting of a precondition, a transformation, and a postcondition. The precondition checks whether a code fragment can be transformed, the transformation optimizes the code fragment to a new form, and the postcondition specifies the properties of the transformed code.
Inverting the optimization means that the postcondition of \opt becomes the precondition of \deopt, \ie, checking whether a code fragment has been optimized by \opt. The transformation of \deopt is derived by inverting the transformation of \opt. The precondition of \opt becomes the postcondition of \deopt, specifying the result of deoptimization.
% Although the postcondition of \deopt is not equivalent to the precondition of $opt$, this does not compromise our method. This discrepancy is acceptable because the postcondition of \deopt is not required in the subsequent steps.

It is worth noting that inverting the transformation is non-trivial.
Compiler optimization often involves multiple-to-one mappings, where multiple distinct programs can be optimized into the same program. Consequently, our deoptimization cannot precisely recover the original program from an optimized version. Despite this, it does not imply that we can invert optimizations without any restriction. 
Instead, we must over-approximately design the inversion \st the following property holds: given an \opt and a program $P$ without undefined behaviors, if $P$ is transformed to $P_o$ by \opt, when we apply \deopt to $P_o$ (resulting in $P_o'$), then $P_o'$ can be optimized by \opt. 
Formally, we define the following property:
\begin{definition}[Re-optimiable]
	\label{def:reopt}
	% Given an optimization $opt$ and a program $P$ without undefined behaviors, if $P$ is optimized to $P_o$ by $opt$, then when we apply $deopt$ to $P_o$ (resulting in $P_d$), the \textit{TODO} property holds when $P_d$ can be re-optimized by $opt$.
	%	Given a deoptimization $deopt$ inverted from $opt$ and a program $P$ without undefined behaviors, a deoptimization $deopt$ satisfies the \textit{Reoptimiable} property when we deoptimize $P$ by $deopt$ to produce $P'$, $P'$ is guaranteed to satisfy the precondition of $opt$.
	Given a deoptimization \deopt inverted from \opt and programs $\mathcal{P}$ without undefined behaviors,  $deopt$ satisfies the \textit{Re-optimiable} property when the following requirement holds:
	$$
    \frac
    {
    \begin{array}{c}
        \forall P \in \mathcal{P}, P' = deopt(P)
    \end{array}
    }
    {
    \begin{array}{c}
        P' \text{satisfies the precondition of }\opt \\
    \end{array}
    }
	$$
\end{definition}
Although the postcondition of \deopt is inequivalent to the precondition of \opt, this does not undermine our method. This discrepancy is acceptable because we do not require the postcondition of \deopt in the subsequent steps.


% % With this property, $P'$ is guaranteed to be optimizable by $opt$ because $P'$ satisfies the precondition of $opt$.
% % The reason for introducing this properly is that our approach reflects the semantics of counterproductive. 
% % Specifically, given a program $P'$, we can say that it is possible for a developer to manually optimize $P'$ to $P$ by applying $opt$.
% % Then, when we found that $P'$ outperforms $P$, we can claim that we found a counterproductive bug. 
% % Otherwise, we cannot draw the conclusion because $P'$ might not be optimized by $opt$.

% According to this property, $P'$ is guaranteed to be optimizable by \opt because $P'$ satisfies the precondition of \opt.
% % The reason for introducing this property is to capture the semantics of counterproductive optimizations.
% The reason for introducing this property is to simulate the scenario of finding compiler defects that lead to the mishandling of developers' optimizations.
% Specifically, with this property, it is possible for a developer to manually optimize the deoptimized program $P'$ to $P$ by applying \opt.
% If we then find that $P'$ outperforms $P$, we can conclude that we have identified a mishandling defect.
% Otherwise, we cannot make this conclusion because, without this property, developers cannot optimize $P'$ to $P$ by \opt, which invalidates our approach.


% Following our deoptimization procedure, we design a list of deoptimizations, which are shown in 
Table~\ref{table:transforms} shows the list of deoptimizations we design. All the deoptimizations are inverted from optimizations selected according to our proposed criteria. Specifically, these optimizations modify the instructions and structure of the original program and thus impact various compiler optimization components, including control flow, memory, and arithmetic optimizations. In addition, they are also common and natural, representing the set of optimizations that developers often apply to reduce code size or improve runtime performance in real-world programming.

We take \textit{InstExpand} as an example. The name \textit{InstExpand} is derived from \textit{InstCombine}, an arithmetic optimization designed to reduce the number of instructions, memory accesses, or execution time required for arithmetic computations while preserving the program's correctness. 
The optimization transforms \myinline{a && b} to \myinline{!(!a || !b)}, where \myinline{a} and \myinline{b} are two variables. The precondition, transformation, and postcondition of this optimization are \myinline{a && b}, \myinline{a && b} $\rightarrow$ \myinline{!(!a || !b)}, and \myinline{!(!a || !b)}, respectively. According to the inversion method, the precondition of the deoptimization is \myinline{!(!a || !b)}, and the transformation is inverted from \myinline{a && b} $\rightarrow$ \myinline{!(!a || !b)} to \myinline{!(!a || !b)} $\rightarrow$ \myinline{a && b}.

% As arithmetic optimizations consist of various optimizations, we show an optimization that transforms \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} to  \myinline{A | B}, where \myinline{A} and \myinline{B} are two variables. 
% The precondition, transformation, and postcondition of the optimization are  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)},  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} $\rightarrow$   \myinline{A | B}, and \myinline{A | B}, respectively. According to our inversion method, we invert the optimization from \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} $\rightarrow$   \myinline{A | B} to \myinline{A | B} $\rightarrow$  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)}, resulting a new deoptimization.  
% After selecting the optimization, we invert the optimization procedure from \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} $\rightarrow$   \myinline{A | B} to \myinline{A | B} $\rightarrow$  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)}, resulting a new deoptimization.  \wyc{explain it by the previous paragraph.}
% \ke{what optimizations do you choose and do not choose why? Cite dragon book, 
% then go to specific examples data-flow, control-flow} resolved

\begin{table*}
	\caption{A list of deoptimizations. \wyc{check against syntax.}}
	\centering
 \adjustbox{max width=1\textwidth}{
	\begin{tabular}{ | c | c | c | }
		\hline
		Name                       & Description                                           & Example                   \\
		\hline
		\textit{InstExpand}        & \tabincell{c}{Make instructions \\ more complex}                        &

		\begin{minipage}[m]{0.75\textwidth}
			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/instexpand.c}
		\end{minipage}
		\\
		\hline
		\textit{CFGExpand}         & \tabincell{c}{Make control-flow\\ more complex}                        &
		\begin{minipage}[m]{0.75\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/cfgexpand.c}

		\end{minipage}
		\\
		\hline
		\textit{Reassociation} & \tabincell{c}{Reassociate \\expressions randomly }                     &
		\begin{minipage}[m]{0.75\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/reassociate.c}

		\end{minipage}
		\\
		\hline
  %SIMD
		\textit{Scalarizing}  & \tabincell{c}{Scalarize the SIMD \\(Single Instruction/\\Multiple Data) \\ operations} & \begin{minipage}[m]{0.75\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/scalarize.c}

		\end{minipage}
		\\
		\hline
		\textit{Dehoisting}    & \tabincell{c}{Put loop-invariants \\into loops  }                      & \begin{minipage}[m]{0.75\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/loopsink.c}

		\end{minipage}
		\\
		\hline
		% \textit{RandomSink}        & \tabincell{c}{Randomly sink instructions                                          \\to different basic blocks} &

		% \begin{minipage}[m]{0.55\textwidth}

		% 	\lstset{style=mystyle, numbers = none, xleftmargin=2em,frame=none}
		% 	\lstinputlisting[]{./code/mutation/sink.c}

		% \end{minipage}
		% \\
		% \hline
		% \textit{RandomMem2Reg}     & Promote stack to register                            &
		% \begin{minipage}[m]{0.55\textwidth}

		% 	\lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=none}
		% 	\lstinputlisting[]{./code/mutation/mem2reg.c}

		% \end{minipage}
		% \\
		% \hline
		\textit{Reg2Mem}     & \tabincell{c}{Demote register \\to stack}                              &
		\begin{minipage}[m]{0.75\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/reg2mem.c}
			% \hline
		\end{minipage}
		\\
		\hline
		\tabincell{c}{\textit{DeadCode-}\\\textit{Insertion}}    & \tabincell{c}{Randomly insert\\ dead code }                            &
		\begin{minipage}[m]{0.75\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/dead.c}

		\end{minipage}
		\\
		\hline
          \begin{tabular}{@{}c@{}}\textit{DeadStore-} \\ \textit{Manipulation}\end{tabular} & \tabincell{c}{Insert dead \\store and move\\ stores around }                        &
		\begin{minipage}[m]{0.75\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/clobber.c}

		\end{minipage}
		\\
		\hline
	\end{tabular}}
	\label{table:transforms}
\end{table*}

\subsubsection{Designing Optimization-Irrelevant Transformations.}
\wyc{todo: revise again.} \wyc{todo: Optimization Obstruction?}
To construct optimization-irrelevant transformations,  we take into account the following criteria:
\begin{itemize}[leftmargin=*]
	\item \textbf{Simplicity}. We define each transformation to be a simple, semantically-preserving transformation by itself such that we do not require a deeper analysis to obtain the guarantee of the semantic equivalence between the original program and the transformed program.
	\item \textbf{Generality}. We define each transformation to be general and widely applicable such that they together can induce a considerable number of semantically equivalent programs to any input.	
	\item \textbf{Diversity}.  We define transformations to produce different types of changes (\eg, insertion and substitution) on different parts of an input program (\eg, variables, operators, and statements) such that generated programs are manifested in diverse forms.
\end{itemize}
Table~\ref{table:oit} shows the list of optimization-irrelevant transformations we design. All the transformations are designed according to our proposed criteria. 
We take \textit{Statements permutation} as an example. The transformation swaps the order of two statements in the code. Note that we will analyze the dependency between the two statements before swapping the two statements. Statements can be swapped only if there is no dependency between them.


\begin{table}
	\captionsetup{skip=2pt}
	\caption{Optimization-irrelevant transformation used in this paper.}
	\label{table:oit}
	\centering
 \adjustbox{max width=1\textwidth}{
		\begin{tabular}{ c|c|c}
			\hline
			\makebox[.14\textwidth][c]{Name} & \makebox[.4\textwidth][c]{Description} & \makebox[.3\textwidth][c]{Example} \\\hline 
			\textbf{Renaming} &
				\begin{tabular}{@{}p{.34\textwidth}} Replace names of variables with common variable names randomly selected from other programs.\end{tabular} & \begin{minipage}[m]{0.5\textwidth}
			\lstset{style=mystyle, frame=none} \begin{lstlisting}
//before:
f(int length){size=length+1;}
//after:
f(int funcName){size=funcName+1;}\end{lstlisting}
		\end{minipage}
	\\\hline  
			
			\textbf{\tabincell{c}{Statements\\permutation}} & \begin{tabular}{@{}p{.34\textwidth}} Permute two statements without data and control dependency.\end{tabular} &
 \begin{minipage}[m]{0.5\textwidth}
			\lstset{style=mystyle, frame=none} \begin{lstlisting}
//before:       //after:
int n=1;        int m=length;
int m=length;   int n=1;\end{lstlisting}
		\end{minipage}
			\\\hline
			\textbf{\tabincell{c}{Operands\\permutation}}& \begin{tabular}{@{}p{.34\textwidth}} Permute two operands of binary operations satisfying the commutative law.\end{tabular} & 	\begin{minipage}[m]{0.5\textwidth}
\lstset{style=mystyle, frame=none} 
\begin{lstlisting}
//before:       //after:
r=a+b;          r=b+a;\end{lstlisting}
		\end{minipage}\\\hline
			\textbf{\tabincell{c}{Operators\\toggling}}& \begin{tabular}{@{}p{.34\textwidth}}Toggle arithmetical operators associated with variables.\end{tabular} &
 \begin{minipage}[m]{0.5\textwidth}
\lstset{style=mystyle, frame=none} \begin{lstlisting}
//before:       //after:
d=a-b+c;        d=a-(b-c);\end{lstlisting}
		\end{minipage}\\\hline
			\textbf{\tabincell{c}{Boolean\\negation}}&  \begin{tabular}{@{}p{.34\textwidth}} Negate the value of a boolean variable, and propagates this change in the program to ensure a semantic equivalence of the transformed program. \end{tabular}&
 \begin{minipage}[m]{0.5\textwidth}
\lstset{style=mystyle, frame=none} \begin{lstlisting}
//before:
boolean flag=true;
if (flag){...}
//after:
boolean flag=false;
if (!flag){...}\end{lstlisting}
		\end{minipage}\\\hline
			\textbf{\tabincell{c}{Branch\\rewriting}}&  \begin{tabular}{@{}p{.34\textwidth}} Replace a \texttt{switch} statement with \texttt{if} statements or vice versa. If the branch is a if-then-else statement, we replace it with a ternary conditional operator or vice versa.\end{tabular} &
 \begin{minipage}[m]{0.5\textwidth}
\lstset{style=mystyle, frame=none} \begin{lstlisting}
//before:
switch(n){
case 1: r=a; break;
case 2: r=b; break; ...
//after:
if(n==1) r=a;
else if(n==2) r=b; ...\end{lstlisting}
		\end{minipage}\\\hline
			\textbf{\tabincell{c}{Loop\\rewriting}}&  \begin{tabular}{@{}p{.34\textwidth}} Replace \texttt{for} loops with \texttt{while} loops or vice versa.\end{tabular} & 
\begin{minipage}[m]{0.5\textwidth}
\lstset{style=mystyle, frame=none} \begin{lstlisting}
//before:
for(int i=0;i<n;i++){...}
//after:
int i=0; while(i<n){...;i++}\end{lstlisting}
		\end{minipage}
  \\\hline
			\textbf{\tabincell{c}{Expression\\unfolding}} & \begin{tabular}{@{}p{.34\textwidth}}Replace expression with a single variable, with common variable name, holding the computed value.\end{tabular} &
 \begin{minipage}[m]{0.5\textwidth}
\lstset{style=mystyle, frame=none} 
\begin{lstlisting}
//before:
Math.min(values.length, length);
//after:
int var=values.length; 
Math.min(var,length);\end{lstlisting}
		\end{minipage} \\\hline 
			\textbf{\tabincell{c}{Deadcode\\insertion}} & \begin{tabular}{@{}p{.34\textwidth}}Insert code into branches or loops whose condition are always evaluated to false. \end{tabular} &
 \begin{minipage}[m]{0.5\textwidth}
\lstset{style=mystyle, frame=none} 
\begin{lstlisting}
//before:
int i = Math.random();
//after:
int i = Math.random(), j = i * i;
if(j < 0) {/* deadcode */}\end{lstlisting}
		\end{minipage} \\\hline
		\end{tabular}}
	\vspace*{-13pt}
\end{table}

\subsubsection{Applying Universal Transformations}
% The diversity of test cases is critical to most testing approaches~\cite{hemmati2013achieving}.
% In order to enhance the diversity of our deoptimized programs, we choose random testing~\cite{hamlet1994random} since it has been proven to be effective in various testing tasks~\cite{huang2019survey}.
After constructing universal transformations, the next step is using them to generate new programs. Concerning the diversity of the generated programs, we balance the frequency of the application of each universal transformation. This ensures every single transformation has contributed to the generation of some transformed programs.
 % second, we cap the total number of deoptimizations applied to the original program at no more than three. Applying deoptimizations too many times could result in overly artificial code, for which compilers are unlikely to generate more efficient code than they do for original programs. Because, ultimately, compilers are not designed to optimize fringe programs that do not resemble those that developers write in the real-world.




% We choose to randomly apply deoptimization 
% % since this strategy has been proven to be effective in various testing tasks~\cite{huang2019survey, humbatova2021deepcrime}
% Technically, we first randomly select a set of deoptimizations $deopt_i$ from Table~\ref{table:transforms}.
% Then, we randomly order these deoptimizations, forming a deoptimization sequence $(deopt_{n})_{n\in\mathbb{N}}$.
% This sequence transforms the original program $P$ into a new program $P'$. Even though $P'$ seems completely different from $P$, it maintains the same functionalities and semantics.


% \subsection{Compiler Optimization}
% \wyc{To Discuss: should we add compiler optimization discussion? i.e., Therefore, the seed program $P$ is optimized to $P_O$ at an optimization level (\eg, \textit{O3}), while the mutated program $P'$ is optimized to $P'_O$ at the same or lower optimization level (\eg, \textit{O3} or \textit{O2}). }

% In this component, we optimize the input program $P$ and the deoptimized program $P'$ respectively. 
% The core component of the compiler under tested in this article is the optimization module, which transforms one program into another more efficient program and preserves the semantics. 
% We expect the tested compiler to generate optimized programs with comparable performance after compiling equivalent programs. 
% Therefore, the seed program $P$ is optimized to $P_O$ at the \textit{O3} optimization level, while the mutated program $P'$ is optimized to $P'_O$ at the same \textit{O3} optimization level. In this way, each optimized program serves as a mirror for the other.

\subsection{Phase Ordering}
After applying universal transformations, the next step is to find the best optimization sequence from a finite set of program optimizations.
The naive iterative compilation approach simpily exhaustively enumerate all possible combination of optimizations, which is too expensive for real-world programs. 
Recent phase ordering approaches can be categorized into three types: iterative compilation and machine learning-based optimization sequence prediction.
% Recent work mainly focus on machine learning approaches~\cite{xxx, xxx}, because exhaustive enumeration is usually infeasible for real-world programs.

In order to demonstrate the benefit of using \prob instead of \spo{}, we choose the state-of-the-art methods for both types of phase ordering approaches. Because we can evaluate the efficiency of finding the optimal program and the efficiency of the optimal program for both kinds of methods.

\subsubsection{Iterative Compilation Approach}
% Recently, some work present some heuristics to reduce the time in finding the optimal sequences, while they cannot guarantee to find the global optimal sequence~\cite{nobre2016graph, kulkarni2009practical, purini2013finding}. 
In iterative compilation techniques, a heuristic search algorithm is used to prune the optimization sequence space to converge onto a good sequence. 
Although they can reduce the time in finding the optimal sequences, they cannot guarantee to find the global optimal sequence~\cite{nobre2016graph, kulkarni2009practical, purini2013finding, kulkarni2006exhaustive}. 
%Even for very good heuristic techniques, the number of required program evaluations would be prohibitively large to use in nontrivial application programs.

~\citet{nobre2016graph} presented an iterative approach to the phase ordering problem using a graph that compiler experts manually constructed based on their knowledge of compiler pass interdependence.
~\citet{kulkarni2009practical} employed techniques to prune the phase order search space in a compiler and utilized estimation techniques to minimize the number of simulations while identifying the optimal performing function instance. 
Instead of searching for a single universally optimal sequence, ~\citet{purini2013finding} construct a small set of good sequences such that for every program class there exists a near-optimal optimization sequence in the good sequences set. Then, they choose the best sequence for a program by trying all the sequences in the good sequences set.

In this experiment, we choose the phase ordering method from~\citet{purini2013finding}, because it is the most recent work that achieves state-of-the-art performance and can automate the whole phase ordering process. In contrast, the method proposed by \citet{nobre2016graph} requires manually constructing a graph for optimizations.


\subsubsection{Machine Learning Approach}
In the machine learning-based approach, the parameters of a chosen prediction model are learned during an offline training phase by observing the runtimes of a set of sample programs optimized using randomly selected sequences. The prediction model is then used to determine the set of optimizations that should be enabled for a given source program. A compiler-specific default ordering for the enabled optimizations is subsequently used to optimize the program.


~\citet{9306994} propose a deep reinforcement learning approach to optimize LLVM's O3 sequence.
~\citet{haj2020autophase} propose a deep reinforcement learning framework, instantiated in the LLVM compiler context for high-level synthesis programs, to find optimal pass sequences. 
~\citet{kulkarni2012mitigating}  propose a novel approach using neuro-evolution to construct an artificial neural network that predicts beneficial optimization orderings on a per-method basis within a dynamic compiler. 

In this experiment, we choose the phase ordering method from~\citet{haj2020autophase}, because it is the most recent machine learning based work and achieves state-of-the-art performance among related works.


\subsection{Overall Algorithm}
Algorithm~\ref{alg:cc} depicts our overall algorithm. Given the original program \po{}, we exhaustively enumerate all possible sequences of universal transformations (line~\ref{line:cc:enuD}). Then, for each transformation sequence $s_1$, we apply $s_1$ to \po{} to generate transformed programs $P_1$ (line~\ref{line:cc:de}). We use the existing phase ordering method to find the global optimal program $P_2$ for $P_1$ (line~\ref{line:cc:po}). If $P_2$ outperforms existing program $P_o'$, we save $P_2$ as $P_o'$ and record its performance (lines~\ref{line:cc:pocheckstart} to~\ref{line:cc:pocheckend}).
Finally, the algorithm returns the most optimal program it can find (line~\ref{line:cc:ret}).
It is worth noting that the existing phase ordering method can be any existing work. \textit{PhaseOrdering} function in the algorithm depicts an exhaustive approach.

\begin{algorithm}[t]
	% \footnotesize
	% \captionsetup{font=scriptsize}
	\algnewcommand\Ins{$I$\xspace}
	\algnewcommand\OP{\poc}
	\algnewcommand\Prog{$P$\xspace}
	\algnewcommand\pdd{\ensuremath{P_1}\xspace}
	\algnewcommand\poo{\ensuremath{P_2}\xspace}
	\algnewcommand\DP{\pdc}
	\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}

	\caption{Finding the global optimal program by \prob.}
	\label{alg:cc}
	\begin{algorithmic}[1]
		\Procedure{FindDefects}{\po}
        \State \pd $\gets$ \po{}, $T \gets t(\pd)$\label{line:cc:destart} 
		\State $\mathcal{S}_D$ $\gets$ \textit{enumerateTransformations}($\mathcal{D}$) \label{line:cc:enuD} 
		\For{$s_1$ \textbf{in} $\mathcal{S}_D$}
	         \State \pdd $\gets$ $s_1(\pd)$ \label{line:cc:de}
			 \State \poo $\gets$ \Call{PhaseOrdering}{\pdd, $\mathcal{O}$} \label{line:cc:po}
				\If{$t(\poo) > T$}  \label{line:cc:pocheckstart}
				\State  \pd $\gets$ \poo, $T \gets t(\poo)$
				\EndIf \label{line:cc:pocheckend}
		\EndFor\label{line:cc:deend}
		\State  \Return{\pd} \label{line:cc:ret}
		\EndProcedure
		
		\item[]

		\Function{PhaseOrdering}{\pdd, $\mathcal{O}$}
        \State \pd $\gets$ \pdd, $T \gets t(\pdd)$\label{line:cc:destart} 
		\State $\mathcal{S}_O$ $\gets$ \textit{enumerateTransformations}($\mathcal{O}$)
		\For{$s_2$ \textbf{in} $\mathcal{S}_O$}
		   \State \poo $\gets$ $s_2(\pdd)$ \label{line:cc:de}
		   \If{$t(\poo) > T$}  \label{line:ifstart}
		   \State  \pd $\gets$ \poo, $T \gets t(\poo)$
		   \EndIf \label{line:cc:ifend}
	   \EndFor\label{line:cc:deend}
	   \State  \Return{\pd} \label{line:cc:ret2}
		\EndFunction
	\end{algorithmic}
\end{algorithm}

==> formalize.tex <==
\section{Background}
\wyc{todo: may pick existing work as background.}


\section{Formalization}
\label{sec:form}


In this section, we define our problem and discuss its properties. 


\subsection{Syntax of Language}


% Throughout the paper, we assume that optimizations implemented by developers manually fall within the broader set of optimizations performed by compilers. In other words, any optimization that developers apply at the source code level can be applied by compilers at the intermediate representation or machine code levels. 
To present our approach formally, we use the call-by-value language shown in Figure~\ref{fig:programsyntax}, similar to the previous work~\cite{shi2018pinpoint, dillig2011precise}:

\begin{figure}[t]
	\centering
	\scalebox{0.9}{
  %     \ovalbox{
	  $
	  \begin{array}{c@{\hspace{.5cm}}rll}
		\mbox{Program P} & \coloneq& F^+ \\
	  \mbox{Function F} & \coloneq & f(v_1, v_2, \dots) \{S;\} \\
		  \mbox{Statement S}  & \coloneq & S_1; S_2 \mid  v_1 \gets v_2 \mid v \gets \phi(v_1, v_2, \dots) \mid v_1 \gets v_2 \; binop \; v_3 \mid  \\
		  &  & v_1 \gets \; unop \; v_3 \mid v1 \gets *(v_2, k \in \mathbb{N}^+) \mid *(v_1, k\in \mathbb{N}^+) \gets v_2  \mid \\
		  &  & if (v) \; then \; S_1; \; else \; S_2 \mid \textbf{return}\; v \mid r \gets call \; f(v_1, v_2, \dots) \\
		  \textbf{binop}  & \coloneq & + \mid  - \mid \wedge \mid \vee  >   \mid  = \mid \neq  \mid \dots \\
		  \textbf{unop}& \coloneq & - \mid \neg \mid \dots  \\
	  \end{array}
	  $}
   % }
	\caption{Program Syntax}
	\label{fig:programsyntax}
\end{figure}

\subsection{Program Definition}

Our focus is on how to find the optimal program, so the first issue is how to determine whether a program is more optimal than another one.
Here, we use function $t$ to measure the performance of a program by existing oracle (\eg, running time, processor clock cycles, code size).
The lower $t(P)$, the higher the program's performance $P$. 
The basic property of the performance measurement function $t$ is decidable.
Based on $t$, we introduce the \opo{}~\cite{touati2006decidability}.
% Here, we use function $t$ to measure the execution time (in processor clock cycles)~\cite{touati2006decidability}. Formally,
% \begin{definition}[Execution Time]
% 	\label{def:et}
%     $\forall P \in \mathcal{P}, \forall I \in \mathcal{I}$, where $\mathcal{P}$ denotes a set of all programs from a programming language. $t(P, I)$ produces processor clock cycles of program $P$ for input $I$.  
% \end{definition}
% On the basis of Definition~\ref{def:et}, we introduce the existing \opo{}~\cite{touati2006decidability}.


\begin{definition}[\opo{}]
	\label{def:po}
    Let $\mathcal{M}$ be a finite set of semantics-preserving transformations. $\forall T \in \mathbb{N}$ an execution time, $\forall P$ a
program, $\forall I$ input data, does there exist a sequence $s \in \mathcal{M}^*$ such
that $t(s(P), I) < T$? In other words, if we define the set:
$$\mathcal{S}_{t,\mathcal{M}}(P, I, T ) = \{s \in \mathcal{M}^*|t(s(P), I) < T \}$$
is the set $\mathcal{S}_{t,\mathcal{M}}(P, I, T ) = \emptyset$ ?
\end{definition}

Textually, the \opo{} problem tries to determine for each program and input whether there exists or not a compilation sequence $s$ which results in an execution time lower than a bound $T$.
It is worth noting that the definition is different from recent work that focuses on the problem of selecting the best set of program transformations to find the global optimal program~\cite{ashouri2017micomp}.
However, the two definitions are equivalent because Definition~\ref{def:po} can be transformed into the problem of finding the global optimal program in polynomial time. \wyc{add a proof?}
We discuss a basic property of Definiton~\ref{def:po} --- it covers the global optimal programs.

\begin{theorem}[The Existence of The Global Optima]
    \label{theo:global}
    Given a program $P_o$, and a program set $\mathcal{P}_{P_o}$ whose elements are all semantically equivalent to $P_o$. There exists a global optimal program $P_o' \in \mathcal{P}_{P_o}$, \st $\forall P \in \mathcal{P}_{P_o}$, $t(P) \geq t(P_o')$.  \wyc{todo: definition of semantically equivalent? use alex aiken's paper?}
\end{theorem}

\begin{proof}
	Assume additionally for the sake of contradiction that $P_o'$ does not exist. It implies that $\forall P_o' \in \mathcal{P}_{P_o}$, $\exists P \in \mathcal{P}_{P_o}$, $t(P) < t(P_o')$. 
	If $\mathcal{P}_{P_o}$ is finite, then we can construct a program by exhaustively enumerating all $P \in \mathcal{P}_{P_o}$ and find $P_o'$ with the smallest $t(P_o')$. The program $P_o'$ is the global optima. 
	On the other hand, if $\mathcal{P}_{P_o}$ is infinite, then although we cannot find the global optima by enumerating $P \in \mathcal{P}_{P_o}$, it is clear that for the program $P_o$, $\exists P_0 \in \mathcal{P}_{P_o}$ \st $t(P_0) < t(P_o)$. We can always find a program $P_i, i\in \mathbb{N}^+$, \st, $t(P_i) < t(P_{i-1})$. However, this procedure cannot do forever because $t(P) \in \mathbb{N}$. Thus, $t(P)$ has a lower bound, so we can find a program $P_o'$ with $t(P_o')$ that equals the lower bound.  Then, the program $P_o'$ satisfies the condition: $\forall P \in \mathcal{P}_{P_o}$, $t(P) \geq t(P_o')$. 
	We can see that both cases contradict the assumption that $P_o'$ does not exist.
	Therefore, we prove that the global optimal for programs that are semantically equivalent to $P_o$ exists.
	% Assume additionally for the sake of contradiction that $P_o'$ does not exist. Then we consider two cases. The first case is $\exists P \in \mathcal{P}, t(P) < t(P_o)$, we can find a global optimal by iteratively applying the \opo{} problem on $P$ when $T = t(P)$. On the other hand, if $\forall P \in \mathcal{P}, t(P) \geq t(P_o)$, then $P_o$ itself is the global optima. Both cases contradict to the assumption that the global optimal program does not exist. Therefore, the \opo{} problem has the global optima.
	%Then $\exists P \in \mathcal{P}$ that $P$ is more efficient than $P_o'$. Then, $P$ is a new global optimal program, indicating that the global optima still exists, which contradicts the assumption. So $P_o'$ exists. 
\end{proof}

% Even though the global optima exists in the \opo{} problem, the problem is undecidable~\cite{touati2006decidability}. Moreover, this problem is not practical in real-world programs. 
Even though the global optima exists in the \opo{}, the problem is not practical in real-world programs. 
Because compiler developers design compiler optimization by a widely-accepted principle --- optimizations should reduce the execution time of a program. 
Recent literature mainly focuses on the \opo{} closely related to selecting the best set of existing compiler optimizations in a fixed ordering~\cite{ashouri2018survey, xxx, xxx}. 
% We summarize these problems and present the \spo{} problem.
Therefore, we introduce an additional constraint to the \opo{}, where any optimization should increase the level of efficiency. We introduce the level of efficiency, a key premise on compiler optimizations, in Definition~\ref{def:loe}.

\begin{definition}[Levels of Efficiency]
	\label{def:loe}
    Let $\mathcal{O}$ be the entire set of optimizations a compiler can perform. Let $m: \mathcal{P} \rightarrow \mathcal{P}$ be one optimization (\ie, $m \in \mathcal{O}$) which takes an input program $P$ and produces an output program $P'$. $P'$ is said to be more efficient than $P$ \textit{iff} $P'$ can be obtained by transforming $P$ using an arbitrary number of optimizations in $\mathcal{O}$, denoted by $P' = s(P)$ where $m \in \mathcal{O}^*$. %\wyc{more efficient or not less efficient? but have to be more efficient, otherwise the next definition has infinite programs.}
\end{definition}

On the basis of the level of efficiency, we additionally assign each transformation a cost, measured by a cost function $c$, in order to be more practical. Because project developers cannot give \opo{} infinite time to search for the global optimal solution.
Such cost may be the transformation time, the number of distinct transformation passes inside a transformation sequence, the length of a transformation sequence, distinct explored transformation sequences, \etc
The problem including the cost function becomes the problem of computing the best transformation sequence within a bounded cost.
The cost function has two inputs: the program $P$ and a transformation pass $m$. So $c$ does not depend on any program input. 
$c(P, m)$ gives the cost of transforming the program $P$ to $P' = m(P)$. 
Finally, we present a \spo{} problem in Definition~\ref{def:spo}: 

\wyc{todo: add a cost function to the following definition, two sequences in \prob should have an overall $K$, instead of two thresholds. }



\begin{definition}[\spo{}]
	\label{def:spo}
    Let $\mathcal{O}$ be a finite set of program optimization that satisfies Definition~\ref{def:loe}.
	Let $c(P, m)$ be a function that computes the cost of transforming the program $P$ to $P'$ = $m(P), m \in \mathcal{O}$
	$\forall T \in \mathbb{N}$ an execution time, 
	$\forall K \in \mathbb{N}$ a computation cost, 
	$\forall P$ a program, $\forall I$ input data, 
	does there exist a sequence $s = (m_n^\frown m_{n-1} \dots ^\frown m_{0})  \in \mathcal{O}^*$ such that $t(s(P), I) < T$ with $\sum_{m_i \in s}^{} c(m_{i-1}^\frown m_{i-2} \dots ^\frown m_0(P), m_i) \leq K $? 
	% In other words, if we define the set: $$\mathcal{S}_{t,\mathcal{O}}(P, I, T ) = \{s \in \mathcal{O}^*|t(s(P), I) < T \}$$ is the set $\mathcal{S}_{t,\mathcal{O}}(P, I, T ) = \emptyset$ ?
\end{definition}

Textually, the \spo{} problem tries to determine for each program and input whether there exists or not an optimization sequence $s$ which results in an execution time lower than a bound $T$. 

% Recent literature mainly focuses on the \spo{} problem~\cite{xxx, xxx, xxx}. Furthermore, most literature~\cite{ashouri2018survey} on the \opo{} is closely related to the problem of selecting the best set of existing compiler optimizations in a fixed ordering.  



The two kinds of \opo{}s have their limitations: (1) the original \opo{} is too difficult; (2) the \spo{} problem only considers optimizations, hindering the program exploration space.  
We discuss the limitation of the \spo{} in detail.
It ignores other semantics-preserving transformations, which may be helpful in finding the global optima. 
Because the number of optimizations in $\mathcal{O}$ in finite, and other semantics-preserving transformations may transform a program $P$ that cannot be optimized by $O \in \mathcal{O}$, into a new program $P'$, while $P'$ can be optimized by $O \in \mathcal{O}$.
We give the example in Figure~\ref{xxx}
\wyc{todo: 1. add example; 2. discuss the drawback in the two \opo{}s.}


To improve the performance of programs found by \opo{}, we present a novel problem, \prob, which finds a transformation sequence for a program before starting \opo{}.
Specifically, we apply transformations other than optimizations (\ie, $\mathcal{D} = \mathcal{M} - \mathcal{O}$) to a program \po, following a cost function $c$. 
Hereinafter, we refer to these transformations as universal transformations.
The cost function is the same as that in Definition~\ref{def:spo}.
When $c(P, m)$ reaches a threshold $K_1$, we obtain a new program \pd, which is guaranteed to be no more efficient than \po. Finally, we send \pd to the \spo{} problem.
Formally, we define the problem in Definiton~\ref{def:prob}.

\begin{definition}[\prob]
	\label{def:prob}
	Let $\mathcal{O}$ be a finite set of program optimization that satisfies Definition~\ref{def:loe}.
	Let $\mathcal{M}$  be a finite set of semantic-preserving program transformations.
    Let $\mathcal{D} = \mathcal{M} - \mathcal{O}$. $\forall T \in \mathbb{N}$ an execution time, $\forall K_1, K_2 \in \mathbb{N}$ a computation cost, $\forall P$ a program, $\forall I$ input data,  $c$ a cost function and $c(P, m)$ gives the cost of transforming the program $P$ to $P' = m(P)$. Does there exist two sequences $s_1 \in \mathcal{D}^*$ and $s_2 \in \mathcal{O}^*$ \st 
	\[ t(s_2(s_1(P)), I) < T, \texttt{ with } \]
	\[ \sum_{m_i \in s_1}^{} c(m_{i-1}^\frown m_{i-2} \dots ^\frown m_1(P), m_i) \leq K_1  \text{ and } \sum_{m_i \in s_2}^{} c(m_{i-1}^\frown m_{i-2} \dots ^\frown m_1(P), m_i) \leq K_2 \]	
% 	In other words, if we define the set:
% $$\mathcal{S}_{t,\mathcal{O}}(P, I, T ) = \{s_2^\frown s_1|s_2 \in \mathcal{O}^*, s_1 \in \mathcal{D}^*, t(s_2(s_1(P)), I) < T,  \sum_{m_i \in s_1}^{} c(m_{i-1}^\frown m_{i-2} \dots ^\frown  m_1(P), m_i) \leq K\}\footnote{$^\frown$ denotes the symbol of sequence concatenation.}$$
% is the set $\mathcal{S}_{t,\mathcal{O}}(P, I, T ) = \emptyset$ ?
\end{definition}

Here we discuss our rationale behind Deﬁnition~\ref{def:prob}. 
We introduce the cost function $c$ to simplify the decision procedure, making \prob also decidable~\cite{touati2006decidability}.
We let $s_1 \in \mathcal{D}^*$ other than $s_1 \in \mathcal{M}^*$ because $s_1 \in \mathcal{M}^*$ makes \prob equivalent to the \opo{} with a cost function but introduces a much wider while unnecessary search space compared to $s_1 \in \mathcal{D}^*$. The search space is unnecessary because \prob also considers optimizations at its second step, which finds transformation sequence $s_2 \in \mathcal{O}^*$. 
% \wyc{todo: the following is important but incorrect, because our following proofs are similar to this one} The search space is unnecessary because $s_1 \in \mathcal{M}^*$ transforms a program $P_o$ into $s_1(P_o)$, if $t(P_o) < t(s_1(P_o))$, we can use $s_2 \in \mathcal{D}^*$ to replace $s_1$. Otherwise, when $t(P_o) \geq t(s_1(P_o))$, we can directly move to the \spo{} and ignore our transformation sequence $s_1 \in \mathcal{D}^*$.

\section{Property}


\subsection{Decidability and Complexity}


% We first prove that \spo{} and \prob are NP problems.

\begin{theorem}[\spo{} is NP]
    \label{theo:sponp}
    \spo{} is an NP problem.
\end{theorem}
\begin{proof}
	The presence of the \spo{} in NP is obvious. Clearly, one can always guess a sequence $s$, verify that it satisfies the constraint for transformation cost, calculate its execution time, and validate whether the execution time is less than $T$ in polynomial time.
\end{proof}

\begin{theorem}[\prob is NP]
    \label{theo:np}
    \prob is an NP problem.
\end{theorem}

\begin{proof}
	The proof is similar to Theorem~\ref{theo:sponp}. We can always guess two sequences $s_1$ and $s_2$, verify that each satisfies its own transformation cost, calculate its execution time, and validate whether the execution time is less than $T$ in polynomial time.
\end{proof}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.99\linewidth]{pics/proofNP.pdf}
	\caption{Reduction to of Knapsack to \prob. All transitions are deterministic. The red arrow shows an example of how we select a transformation sequence.}
	\label{fig:proofnp}
\end{figure}

Now, we introduce OptP and OptP-Complete problem. First, the class of OptP contains optimization problems. These problems involve finding the best solution (maximum or minimum) from a set of possible solutions. Examples include the Traveling Salesperson Problem (TSP), Knapsack Problem, and 0-1 Integer Linear Programming. OptP-Complete refers to a class of computational problems that are challenging to solve. A problem is OptP-complete if it is at least as hard as the hardest problems in the OptP class. For instance, MAX-SAT (finding the lexicographically maximum satisfying assignment) is OptP-complete. The reduction from MAX-SAT to Integer Linear Programming (ILP) shows that ILP is also in OptP.
Compared to NP-complete, OptP-complete is more accurate for our problem. Therefore, we prove that \prob is OptP-Complete~\cite{krentel1986complexity}

\begin{lemma}[\prob is OptP-Complete]
    \label{theo:optp}
    \prob is OptP-Complete.
\end{lemma}

\begin{proof}
	According to Theorem~\ref{theo:np}, \prob is NP. 
	
	We reduce Knapsack problem, an OptP-Complete~\cite{krentel1986complexity}, to \prob problem.
	Recall that Knapsack asks whether, for a given set of items $u \in \mathcal{U}$, each of which has a cost $t(u)$
	and a value $v(u)$, there exists a subset $\mathcal{U}' \subseteq \mathcal{U}$ such that the total value of all items
	in $\mathcal{U}'$ is no less than some constant $W$, and their total cost is no greater than another
	constant $B$, \ie, $\sum_{u \in \mathcal{U}'}^{} t(u) \leq B, \sum_{u \in \mathcal{U}'}^{} v(u) \geq W$.

	Given an instance of Knapsack with $|U| = m$, let us number all items as $u_i, i\in [1,m]$ as a notational convenience. 
	For such an instance of Knapsack, we create a special instance of \prob with a program $P$. 
	% In this instance, we define the performance gain for an optimization as $g = t(P) - t(P')$, where $P'$ is transformed from $P$ by applying the optimization.
	For every item $u_i$ in Knapsack, we define a universal transformation $D_i$ and a bounded optimization $O_i$, where $D_i$ has a cost $t(u_i)$ with zero reward while $O_i$ has a reward $v(u_i)$ with zero cost.
	All $D_i$ (\resp, $O_i$) forms $\mathcal{D}$ (\resp, $\mathcal{O}$).
	We say this is a special instance of \prob problem because we add the following two additional rules:
	(1) $\forall D_i \in \mathcal{D}$, when $D_i$ is selected in $s_1$, its bounded optimization $O_i$ is also selected in $s_2$, with the reversed order as $D_i$ in $s_1$;
	(2) each $ D_i \in \mathcal{D}$ can only be selected once. Note that the second rule implies that each $O_i \in \mathcal{O}$ can only be selected once.

	Figure~\ref{fig:proofnp} shows an example. We follow the red line to illustrate our example. The original program is $P$, if we choose the $m$-th element in $U$, it means that we select $D_m$ to transform $P$ to $P_{<m>}$. Similarly, if we select $m-1$-th element in $U$ to transform $P_{<m>}$, then the resultant program is $P_{<m, m-1>}$. After building the transformation sequence $s_1$ from $\mathcal{D}$, the optimization sequence $s_2$ is automatically constructed by selecting the bounded optimization with the reversed order in $s_1$. For this example,  $s_1 = <D_m, D_{m-1}>$, then $s_2 = <O_{m-1}, O_m>$. 

	The above construction basically allows \prob to choose sequences $s_1$ for a program ($s_2$ can be automatically constructed). Choosing the transformation $D_i$ in $\mathcal{D}$ is equivalent to putting item $u_i$ into the knapsack, while not selecting $D_i$ corresponds to the choice of not including $u_i$ in the knapsack. 
	Therefore, it is clear that there exist two sequences $s_1$ and $s_2$ that the total cost of transformation in $s_1$ and $s_2$ is  $B$ (\ie, $K_1=B$ and $K_2=0$), and the execution time $T$ is $t(P) - W$ if and only if there exists a solution $\mathcal{U}'$ to the instance of Knapsack, where $|U| = m$, the total value of all items in $\mathcal{U}'$ is no less than $W$, and the total cost is no greater than $B$. 
	% Therefore, it is clear that there exist two sequences $s_1$ and $s_2$ that the total cost of transformation in $s_1$ is less than $K_1=B$, the cost $K_2$ in $s_2$ is set to $\infty$ (\ie, ignore the limitation for $K_2$), and the performance gain is larger than $W=t(P) - T$ if and only if there exists a solution $\mathcal{U}'$ to the instance of Knapsack, where $|U| = m$, the total value of all items in $\mathcal{U}'$ is no less than $W$, and the total cost is no greater than $B$. 







	% Given an instance of Knapsack with $|U| = m$, let us number all items as $u_i, i\in [1,m]$ as a notational convenience. 
	% For such an instance of Knapsack, we create \prob with $|\mathcal{D}| = m_1$ and $|\mathcal{O}| = m_2$ where $m=m_1+m_2$.
	% For the first $m_1$ items in Knapsack, we define reward $v(u_i), i \in [1, m_1]$ to be zero, and cost $t(u_i), i \in [1, m_1]$ to be the cost $c$ in \prob.
	% For the remaining items in Knapsack, we define reward $v(u_i), i \in [m_1+1, m]$ to be the performance gain and cost $t(u_i), i \in [m_1+1, m]$ to be zero.
	% We define $B$ in Knapsack as $K$ in \prob, and $W$ in Knapsack as $T$ in \prob.

	
	% The above construction basically allows \prob to search the optimal programs.
	% Choosing a transformation in $\mathcal{D}$ is equivalent to putting an item $u_i, i \in [1, m_1]$ into the Knapsack, while choosing an optimization in $\mathcal{O}$ is equivalent to putting an item $u_i, i \in [m_1+1, m]$ into the Knapsack. 
	% Therefore, we can conclude that there exist two sequences $s_1$ and $s_2$ that satisfy $t(s_2(s_1(P)), I) < T$ and $\sum_{m \in s_1}^{} c(P, m) \leq K $ if and only if there exists a solution to the original instance of Knapsack.
\end{proof}

\begin{lemma}[\prob is NP-Complete]
    \label{theo:npc}
    \prob  is NP-Complete
\end{lemma}

\begin{proof}
	According to Lemma~\ref{theo:optp}, we can conclude that \prob is NP-Complete according to~\citet{krentel1986complexity}.
	\wyc{If we do not need to prove \prob is optp-complete, then the proof is very easy. First, \prob is NP. Second, \prob can be reduced to \opo{}. So \prob is NP-complete.} \wyc{does \opo{} is proved to be np hard? if not, we need a proof.}
\end{proof}


\subsection{The relation between \prob and \opo{}.}

We first discuss a natural but important relationship between \prob and \opo{}, \ie, \prob can find the global optimal program that \opo{} can find.

\begin{theorem}[\prob can find the global optima that \opo{} can find]
    \label{theo:global}
    Given a program $P_o$ and the global optimal program $P_o'$ that is semantically equivalent to $P_o$ while $P_o'$ is found in the \opo{} (Definition~\ref{def:po}), \prob may also be capable of finding a program $P_o''$ where $t(P_o') = t(P_o'')$. 
\end{theorem}

\begin{proof}
	% Assume additionally for the sake of contradiction that \prob cannot find $P_o'$ in any case. Let the optimal program \prob found is $P_o''$ and $\forall P_o \in \mathcal{P}, t(P_o'') > t(P_o')$. However, \prob is a subset of the problem defined in Definition~\ref{def:po} according to Lemma~\ref{theo:sspo}. Therefore, it is possible that $\exists P_o \in \mathcal{P}, t(P_o'') = t(P_o')$.
	The proof is based on construction. In order to find the program $P_o$, we start with the global optimal program \gp found by \opo{}, and we find a program $P_1$ that can be optimized into \gp by an optimization sequence $s_2 \in \mathcal{O}^*$. Then, for $P_1$, we find a program $P_2$ that can be transformed into $P_1$ by a transformation sequence $s_1 \in \mathcal{D}^*$. $P_2$ is exactly the original program $P_o$ we try to find, because $s_2(s_1(P_2)) = P_o''$, and $P_o'' = P_o'$, so $t(s_2(s_1(P_2))) = t(P_o'') = t(P_o')$. 
    In this way, we found a program $P_o$ satisfies $t(P_o'') = t(P_o')$.
	% Therefore, we can find a program $P_o$ satisfies $t(P_o'') = t(P_o')$, which contradicts the assumption that $\forall P_o \in \mathcal{P}, t(P_o'') > t(P_o')$. So $P_o'$ exists.
\end{proof}


% \wyc{what does subset/superset of problems mean? seems uncommon.}
% \begin{lemma}[\prob is a strict subset of the \opo{}]
%     \label{theo:sspo}
%     Given a program $P_o$, \prob and \opo{} respectively find $P_o'$ and $P_o''$, we say \prob is a strict subset of the \opo{} $\iff (t(P_o') \geq t(P_o'')) \land (\exists P_{o1}, t(P_{o1}') > t(P_{o1}'')) $.
% \end{lemma}

% \begin{proof}
% 	We first prove $t(P_o') \geq t(P_o'')$, this is obvious because transformations in \prob are a subset of that in \spo{}. 
% 	Then, we The interaction of \prob is a subset of \opo{}. Because transformations in \prob are a subset of that in \spo{}. 
% \end{proof}

% \begin{lemma}[\prob is a strict superset of the \spo{} problem]
%     \label{theo:ssspo}
%     Given a program $P_o$, \prob and \spo{} respectively find $P_o'$ and $P_o''$, we say \prob is a strict subset of the \spo{} problem $\iff (t(P_o') \leq t(P_o'')) \land (\exists P_{o1}, t(P_{o1}') < t(P_{o1}'')) $.
% \end{lemma}


% \begin{proof}
% 	We consider two cases:
% (1) \prob is neither a subset of \spo{} nor equivalent to \opo{}. This can be proved by Theorem~\ref{theo:inequivalent}.
% (2) \prob is a superset of \spo{}. Because transformations in \prob are a superset of that in \spo{}. 
% \end{proof}

% Then, we discuss in detail the relationship between \prob and the \opo{} --- the subset relation between \prob, \opo{}, and \spo{}. 
% We first begin with the definition to clarify what is the subset of two problems.

% \wyc{todo: use $T(prob, P_o)$ may be better, e.g., $T(\prob, P_o) <= T(\opo{}, P_o)$}
% \begin{definition}[The solution set of a problem]
% 	\label{def:sop}
%     Given a problem $prob$, we use $\mathcal{P}_{P_o}$ to represent all semantically equivalent programs of a program $P_o$, and $prob(P_o)$ to denote the global optimal program found by $prob$. Based on $\mathcal{P}_{P_o}$, we define the solution set of the problem $prob$ as a set of global optimal programs that can be found by $prob$ for a program $P_o$. Formally:
% 	\[ \mathcal{S}(prob, P_o) = \{t(P_o')| P_o'=prob(P_o), \st, \forall P \in \mathcal{P}_{P_o}, t(P_o') \leq t(P) \}\]
% \end{definition}

% \begin{definition}[The solution set of a problem]
% 	\label{def:sop}
%     Given a problem $prob$, we use $\mathcal{P}_{P_o}$ to represent all semantically equivalent programs of a program $P_o$, and $prob(P_o)$ to denote the global optimal program found by $prob$. Based on $\mathcal{P}_{P_o}$, we define the solution set of the problem $prob$ as a set of global optimal programs that can be found by $prob$. Formally:
% 	\[ \mathcal{S}(prob) = \{P_o'| P_o \in \mathcal{P}, P_o'=prob(P_o), \st, \forall P \in \mathcal{P}_{P_o}, t(P_o') \leq t(P) \}\]
% \end{definition}


% \begin{theorem}[\prob is inequivalent to \opo{}]
%     \label{theo:inequivalent}
%     The optimal program $P_{o}'$ found from $P_o$ may be different from $P_{o}''$ found from the original program $s_1(P_o)$ by the same \opo{} approach. 
% 	% Formally, $\exists P_o \in \mathcal {P}, t(P_{o}') \neq t(P_{o}'')$.
% 	Formally,   $\mathcal{S}(\prob) \neq  \mathcal{S}(\text{\opo{}})$.
% \end{theorem}

% \begin{proof} 
% 	This is obvious because \prob is decidable while \opo{} is undecidable. Otherwise, we can use a decidable problem to solve an undecidable problem. \wyc{todo: not sure \opo{} is undecidable.}
% 	% The theorem also means that $\exists P_o, t(s(P_o)) \neq t(s_2(s_1(P_o)))$, where $P_o$ is a program, $s \in \mathcal{M}^*$ (\ie, \opo{}) and $s_1 \in \mathcal{D}^*, s_2 \in \mathcal{O}^*$.
% 	% Assume additionally for the sake of contradiction that for any program $P_o$, then we have $\forall P_o, t(s(P_o)) = t(s_2(s_1(P_o)))$. However, we can construct a program violating the condition. Specifically, we start with a global optimal program \gp where $\forall P \in \mathcal{P}_{\widebar{P_o}}, t(\gp) < t(P)$. We find a program $P_1$ that can be optimized into \gp by a transformation sequence $s \in \mathcal{M}^*$, and $s$ can be split into a set of subsequences $Seq = \{s' \mid s' \in \mathcal{D}^* \lor s' \in \mathcal{O}^*\}$ and $|Seq| > 2$. \wyc{is it true that such $s$ exists?}
% 	% The program $P_1$ is the original program $P_o$ we try to find. We can see that \prob cannot find the global optimal program \gp by finding $s_1 \in \mathcal{D}^*$ and $s_2 \in \mathcal{O}^*$ to transform $P_o$. Therefore, the existence of the program $P_o$ contradicts the assumption that  $\forall P_o, t(s(P_o)) = t(s_2(s_1(P_o)))$. Therefore, we have $\exists P_o, t(s(P_o)) \neq t(s_2(s_1(P_o)))$, which leads to  $\mathcal{S}(\prob) \neq  \mathcal{S}(\text{\opo{}}) $.
% 	% Assume additionally for the sake of contradiction that for any program $P_o$, then it means that the global optimal $P_{o1}'$ found from $P_o$ by \opo{} is the same as $P_{o2}'$ found from the original program $s_1(P_o)$ by \prob, where $s_1$ is an arbitrary transformation sequence from $\mathcal{D}^*$. 
% 	% Then it means that the distribution of execution time for programs $P_o$ is convex, \ie, there exists one and only one global minima. \wyc{seems incorrect.} 
% 	% It is clearly incorrect because two equivalent programs may have the same execution time. 
% \end{proof}

Then, we discuss in detail the relationship between \prob and the two phase ordering problems.

\begin{lemma}[\prob is a subset of \opo{}]
    \label{theo:sspo}
    Given a program $P_o$, \prob and \opo{} respectively find $P_o'$ and $P_o''$, we say \prob is a subset of the \opo{} $\iff \forall P_o \in \mathcal{P}, t(P_o') \geq t(P_o'')$. 
	% We use a simplified form $\mathcal{S}(\prob) \subseteq  \mathcal{S}(\text{\opo{}})$ to represent the relationship.
	% Given a program $P_o$, \prob and \opo{} respectively find $P_o'$ and $P_o''$, we say \prob is a strict subset of the \opo{} $\iff (\forall P_o \in \mathcal{P}, t(P_o') \geq t(P_o'')) \land (\exists P_o \in \mathcal{P}, t(P_{o}') > t(P_{o1}''))$. 
	% We use a simplified form $\mathcal{S}(\prob) \subset  \mathcal{S}(\text{\opo{}})$ to represent the relationship.
\end{lemma}

\begin{proof}
	It is clear that transformation sequences in \prob are a subset of the \opo{}, because \prob only considers optimizations after non-optimizations, while \opo{} is capable of combining any optimizations and non-optimizations in any order. Therefore, with fewer kinds of transformations, \prob can only produce fewer programs, which are also a subset of programs that can be produced by \opo{}. 
    Therefore, \prob is a subset of \opo{}.
	% Moreover,  Theorem~\ref{theo:inequivalent} shows that two problems are inequivalent. Therefore, we have proved \prob is a strict subset of the \opo{}.
\end{proof}


\begin{lemma}[\prob is a superset of \spo{}]
    \label{theo:ssspo}
    Given a program $P_o$, \prob and \spo{} respectively find $P_o'$ and $P_o''$, we say \prob is a superset of the \spo{} problem $\iff \forall P_o \in \mathcal{P}, t(P_o') \leq t(P_o'')$.
	%We use a simplified form $\mathcal{S}(\text{\opo{}}) \subseteq  \mathcal{S}(\prob)$ to represent the relationship.
\end{lemma}
\begin{proof}
The proof is straightforward because \prob first transforms a program into another program, then uses \spo{} to search for the global optimal program.
Specifically, transformations in \prob are a superset of that in \spo{}. With more kinds of transformations, it is impossible to produce fewer programs. 
Therefore, \prob is a superset of \spo{}.
%Therefore, $\mathcal{S}(\text{\opo{}}) \subseteq  \mathcal{S}(\prob)$.
\end{proof}
Although we proved Lemma~\ref{theo:ssspo}, it is an unsurprising property.
In contrast, proving that \prob is a strict superset of the \spo{} problem is more important.
\begin{lemma}[\prob is a strict superset of the \spo{} problem]
    \label{theo:ssspo}
    Given a program $P_o$, \prob and \spo{} respectively find $P_o'$ and $P_o''$, we say \prob is a strict superset of the \spo{} problem $\iff \forall P_o \in \mathcal{P}, t(P_o') \leq t(P_o'') \land (\exists P \in \mathcal{P}, t(P') < t(P'')) $.
\end{lemma}
\begin{proof}
	According to Lemma~\ref{theo:ssspo}, we have proven that \prob is a superset of \spo{}. Consequently, in this proof, we only consider the existence of $P \in \mathcal{P}$ such that $t(P') < t(P'')$.
	The proof of the existence of such a $P$ is based on construction. 
	Initially, \spo{} transforms programs using $\mathcal{O}$, a finite set of program optimizations. 
	In contrast, \prob first transforms programs using $\mathcal{D} = \mathcal{M} - \mathcal{O}$, and then using $\mathcal{O}$. 
	Thus, we can construct a problem $P$ that cannot be optimized by any transformation in $\mathcal{O}$. However, after applying a transformation $m \in \mathcal{D}$ to $P$, the transformed problem $P' = m(P)$ can be optimized by the transformations in $\mathcal{O}$.
	Since our language, defined in Definition~\ref{fig:programsyntax}, is Turing-complete, such a program $P$ does exist.
	Therefore, we have identified a program $P \in \mathcal{P}$, such that $t(P') < t(P'')$.
\end{proof}


% Although we proved Lemma~\ref{theo:ssspo}, it is an uninteresting and unsurprising property.
% In contrast, proving that \prob is a strict superset of the \spo{} problem is more important.
% % Now, we prove that \prob is a strict superset of the \spo{} problem.
% However, with arbitrary cost functions, the property does not hold, because we can design a cost function that assigns any transformations in $\mathcal{D}$ to be an extremely large value, resulting in no $s_1 \in \mathcal{D}^*$ can be applied with a given cost $K_1$. Therefore, \prob is equivalent to the \spo{} problem.

% However, analyzing the scenarios where \prob is a strict superset of \spo{} is critical because we can apply \prob to these scenarios.
% We found that, when we limit the cost function to follow the property defined in Definition~\ref{def:pcf}, we can prove that \prob is a strict superset of the \spo{} problem. 

% \begin{definition}[Restrained cost function]
% 	\label{def:pcf}
%     A cost function $c$ is restrained if and only if $\exists m_1, m_2, m_3 \in \mathcal{O}, \exists m_4 \in \mathcal{D}$, \st $c(m_1) + c(m_2) > c(m_3) + c(m_4)$.
% \end{definition}

% \begin{lemma}[\prob is a strict superset of the \spo{} problem]
%     \label{theo:ssspo}
%      %$\mathcal{S}(\text{\opo{}}) \subset  \mathcal{S}(\prob)$ 
% 	 \prob is a strict superset of the \spo{} problem where $K_1 + K_2 = K$ and the cost function $c$ satisfies Definition~\ref{def:pcf}.
% \end{lemma}
% \begin{proof}
% 	The proofs of Lemma~\ref{theo:ssspo} is based on construction. We begin by finding $m_1, m_2, m_3, m_4$ according to Definition~\ref{def:pcf}.
% 	Then, we find a global optimal program $\gp$, and a program $P_o$ satisfies the following conditions:
% 	\begin{enumerate}
% 		\item $m_2(m_1(P_o)) = m_4(m_3(P_o)) = \gp$;
% 		\item we set the cost bound $K_1 = c(m_3(P_o), m_4), K_2=c(P_o, m_4), K=K_1+K_2$.
% 	\end{enumerate}
% 	For the program $P_o$, the \spo{} cannot find \gp because $K < c(m_1(P_o), m_2) + c(P_o, m_1)$, and thus cannot have enough cost to transformation $P_o$ by $m_2(m_1(P_o))=\gp$. In contrast, \prob can find \gp because $K > c(m_3(P_o), m_4) + c(P_o, m_3)$, and thus cannot have enough cost to transformation $P_o$ by $m_4(m_3(P_o))=\gp$.
% \end{proof}

% \begin{lemma}[\prob is a strict superset of the \spo{} problem]
%     \label{theo:ssspo}
%     Given a program $P_o$, \prob and \spo{} respectively find $P_o'$ and $P_o''$, we say \prob is a superset of the \spo{} problem $\iff \forall P_o \in \mathcal{P}, t(P_o') \leq t(P_o'')$.
% 	$(\forall P_o \in \mathcal{P}, t(P_o') \leq t(P_o'')) \land (\exists P_o \in \mathcal{P}, t(P_{o}') < t(P_{o1}''))$. 
% 	We use a simplified form $\mathcal{S}(\text{\opo{}}) \subset  \mathcal{S}(\prob)$ to represent the relationship.
% \end{lemma}
% \begin{proof}
% The proof is straightforward because \prob first transforms a program into another program, then uses \spo{} to search for the global optimal program.
% Specifically, transformations in \prob are a superset of that in \spo{}. With more kinds of transformations, it is impossible to produce fewer programs. Therefore, $\mathcal{S}(\text{\opo{}}) \subseteq  \mathcal{S}(\prob)$.
% Now, we prove that \prob can find more global optimal programs than \spo{}.
% % To find the program $P_o$, we first randomly select a program $P_1$ and use \spo{} to find the global optimal program \gp.
% % Regarding the probability of finding $P_o \in \mathcal{P}, t(P_{o}') < t(P_{o1}'')$, we can set $K_2 = K$ and $K_1 > \mathbb{N}^+$, where $K_1$ and $K_2$ come from the costs in \prob and $K$ is from the cost in \spo{}.
% % With more cost (\ie, $K_1 + K_2 > K$) to use, 
% To construct the case, we first find a global optimal program $\gp$, and a program $P_1$ that can be optimized into \gp by $s_2(s_1(P_1))$. $s_1$ and $s_2$ satisfies the following conditions:
% \begin{enumerate}
% 	\item $s_1 \in \mathcal{D}^*, s_2 \in \mathcal{O}^*$;
% 	\item the cost of $s_2$ is $K_2$, and the cost of $s_1$ is less than $K_1$.
% 	\item the cost of \spo{} to find \gp from $P=s_2(s_1(P_1))$ is larger than $K$.
% \end{enumerate}
% \wyc{todo: not good}
% The program $P_1$ does exist because we can design the corresponding cost function. Therefore, we construct a program $P_1$ where \prob can find \gp while \spo{} cannot.
% % Since the cost of $s_2$ is $K$, \spo{} cannot find \gp with the cost bounded by $K$ because no cost is left for transforming $P_1$ to $s_1(P_1)$. In contrast, \prob can find it as it is constructed as it is. \wyc{todo}
% \end{proof}

% Although we proved Lemma~\ref{theo:ssspo}, it is an uninteresting property because \prob has more cost to use.
% Now, we prove that \prob is also a strict superset of the \spo{} problem with the same overall cost, \ie, $K_1 + K_2 = K$.
% \begin{lemma}[\prob is a strict superset of the \spo{} problem with the same cost]
%     \label{theo:ssspo}
%      $\mathcal{S}(\text{\opo{}}) \subset  \mathcal{S}(\prob)$ where $K_1 + K_2 = K$.
% \end{lemma}
% \begin{proof}
% 	\wyc{TODO: 	}
% 	Assume additionally for the sake of contradiction that for $\forall P_o \in \mathcal{P}, t(P_o') \geq t(P_o'')$. Since Lemma~\ref{theo:ssspo} has already shown that $\forall P_o \in \mathcal{P}, t(P_o') \leq t(P_o'')$, so we have $\forall P_o \in \mathcal{P}, t(P_o') = t(P_o'')$.
% 	Since $P_o'$ comes from $s_2(s_1(P_o))$ and $P_o''$ comes from $s_2'(P_o)$ where $s_1 \in \mathcal{D}^*$ and $s_2, s_2' \in \mathcal{O}^*$, we have $\forall P_o \in \mathcal{P}, t(s_2(s_1(P_o))) = t(s_2'(P_o))$. 
% 	\wyc{polish:} Since we can use performance-irrelevant transformations $\mathcal{I}$ to represent programs with the same execution time, \ie, $\forall P \in \mathcal{P}, t(P) = t(s(P)), s \in \mathcal{I}^*$.
% 	Furthermore, we can discard the common part between $s_2$ and $s_2'$, resulting in $\bar{s_2}(s_1(P_o))$ and $\bar{s_2'}(P_o)$ where the last transformation in $\bar{s_2}$ and $\bar{s_2'}$ are different. 
% 	The resultant formula is $\forall P_o \in \mathcal{P}, t(\bar{s_2}(s_1(P_o))) = t(\bar{s_2'}(P_o))$.
% 	Moreover, since $t$ can be an arbitrary time measurement function, so $\bar{s_2}$ and $s_1$ can be arbitrary transformations because $t$ can be dedicatedly defined to demonstrate that $\bar{s_2}(s_1(P_o))$ is the global optimal program.
% 	Finally, we use $s \in \mathcal{I}^*$ to replace $t$, leading to $\forall P_o \in \mathcal{P}, \bar{s_2}(s_1(P_o)) = s(\bar{s_2'}(P_o))$.
% 	In summary, we simplify the proof of this theorem into the proof to the following formula:
% 	\begin{equation}
% 		\forall P_o \in \mathcal{P}, \forall s_1 \in \mathcal{D}^*, s_2 \in \mathcal{O}^*, \exists s_3 \in \mathcal{O}^* \text{ and } s_4 \in \mathcal{I}^*, \st, s_2(s_1(P_o)) = s_4(s_3(P_o)). 
% 		\\ \sum_{m \in s_1}^{} c(P, m) \leq K
% 		% Note that the cost of $s_1$ should be less than $K$. 
% 	\end{equation}
% 	% Note that the cost of $s_1$ should be less than $K$. 	Without the constraint, the proof is straightforward because \prob becomes an undecidable problem while \spo{} is decidable.

% \end{proof}




==> method.tex <==
\section{The High-Level Workflow}

In this section, we present a high-level workflow of our approach. 

\subsection{Definitions}

% The new setting that we described in Section~\ref{sec:intro} is simple and intutive. 

% The goal of this subsection is to provide more precise definitions for the new setting 

Throughout the paper, we assume that optimizations implemented by developers manually fall within the broader set of optimizations performed by compilers. In other words, any optimization that developers apply at the source code level can be applied by compilers at the intermediate representation or machine code levels. 

Now, we define the levels of efficiency for programs, which is a key premise for our evaluation on compiler optimizations.

\begin{definition}[Levels of Efficiency]
	\label{def:le}
    Let $\mathcal{O}$ be the entire set of optimizations a compiler can perform. Let $\opt: \mathcal{P} \rightarrow \mathcal{P}$ ($\mathcal{P}$ denotes set of all programs in the universe) be one optimization (\ie, $\opt \in \mathcal{O}$) which takes an input program $P$ and produces an output program $P'$. $P'$ is said to be more efficient than $P$ \textit{iff} $P'$ can be obtained by transforming $P$ using a arbitrary number of optimizations in $\mathcal{O}$, denoted by $P' = \opt^{*}(P)$ where $\opt \in \mathcal{O}$.
\end{definition}

According to Definition~\ref{def:le}, a program that has been optimized by developers manually is more efficient than the original version of the program.



% Now, we present a compiler optimization property.
% \begin{definition}[Monotonicity of Compiler Optimization]
% 	\label{def:moco}
% 	$\forall \opt_i \in \mathcal{OPT}, \, opt(P_i) = P_{i+1}, \, E(P_i) \leq E(P_{i+1})$,
% 	where $\mathcal{OPT}$ is a set of compiler optimizations and $E$ represents the degree of efficiency of a program (with higher values indicating greater efficiency).
% \end{definition}

% This definition leads to our new angle for compiler optimization:
% \begin{definition}[A New Angle for Compiler Optimization]
% 	\label{def:metric}
% 	Any compiler optimization manually made by developers with the intention of enhancing program efficiency should not result in degraded performance.
% \end{definition}

\subsection{Workflow}
Figure~\ref{fig: workflow} depicts the high-level workflow of our approach for finding compiler defects that lead to the mishandling of developers' optimizations. We discuss the major components below:
\begin{itemize}[leftmargin=*]
	\item \textbf{\textit{Original Programs.}}\, Existing studies often opt for programs generated by random code generators (\eg, CSmith~\cite{yang2011finding}) to identify optimization bugs in compilers. However, in this work, we focus on real-world programs, which helps translate our findings to practice more seamlessly. 
	      % in optimization due to fewer redundancies and direct dead parts compared to randomly generated programs, is likely to 
	    %   yield more meaningful real-world contributions.
	\item \textbf{\textit{Deoptimization.}}\, Deoptimizations are critical to our approach. We design deoptimizations by inverting existing compiler optimizations. Then, we apply deoptimizations to the original program \po{}, resulting in a deoptimized program \pd{}.
	\item \textbf{\textit{Compiler Optimization.}}\, We use the compiler under test to optimize both the input program \po{} and the deoptimized program \pd{} using identical compiler optimizations (\eg, O3), generating two compiled codes (denoted as \poc and \pdc).
	      % \item \textbf{\textit{Performance Measurement}}\, We employ static performance checkers to approximate code's runtime efficiency.
	\item \textbf{\textit{Performance Checking.}}\, Our performance checking encompasses two aspects: code size and expected runtime. We employ static performance checkers 
  % to approximate the runtime performance of code and 
    to evaluate whether the deoptimized program \pdc outperforms the original program \poc. If such a situation is observed, we conclude that a mishandling defect has been detected.
	\item \textbf{\textit{Test Case Reduction.}}\, As defects-inducing programs tend to be too large and complex for human developers to understand, we employ automated test-case reduction tool~\cite{lecoeur2023program} to reduce such defects-inducing programs.
	      % a compiler testing setup~\cite{lecoeur2023program}. 
	      %\wyc{to polish} Smaller test cases are more proper for debugging and analysis. By designing an effective test oracle for the automatic test case reducer, we guarantee that the reduced test case maintains counterproductive bugs with the original test case.
\end{itemize}

\vspace*{3pt}
\noindent
\textbf{\textit{Notations.}}\,
We use \po{} (\resp, \pd{}) to denote the original program (\resp, deoptimized program). \poc (\resp, \pdc) represents the code generated by a compiler for \po{} (\resp, \pd{}). If otherwise specified, $P$ denotes a program in the general sense. 
% \wyc{add $R$?}
% \ke{it's fine not a major notation.}


\section{Methodology}

In this section, we present our methodology, in particular, we discuss the major components including deoptimization, performance checking and test case reduction in detail.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.99\linewidth]{pics/workflow.pdf}
	\caption{Overview of our approach.}
	\label{fig:workflow}
\end{figure}

\subsection{Deoptimization}
As explained in Section~\ref{sec:intro}, there are potentially two approaches to generating programs with varying levels of efficiency. Considering our research is centered on real-world programs, which typically offer limited scope for optimization, we choose to deoptimize an original program to produce less efficient variants. In essence, original programs can be viewed as the result of the application of developers' optimizations to deoptimized programs.

Below, we first discuss how to design deoptimizations, and then illustrate how we apply deoptimizations.
% We first introduce basic definitions for deoptimization, then discuss how to design deoptimizations, and finally, we give an algorithm for illustrating how to apply deoptimizations.




% To mutate a given seed program $P$ to $P'$, we design a bunch of semantic-preserving transformations. And assemble them randomly into a pipeline as a mutator.

\subsubsection{Designing Deoptimization}

% To build a deoptimization, we first select an optimization of compilers. Intuitively, we can select any optimization in this phase. 
% In practice, we present a more effective selection criterion: given an optimization pipeline, we analyze which optimization affects which optimization and we choose the top-N strongest optimizations that everyone else depends on~\cite{alfred2007compilers}. 
% It usually suggests that we should avoid selecting optimizations that are irrelevant to data flow or control flow analysis, such as renaming variables. 
% The reason is that our method detects counterproductive bugs by an optimization ``source'': a large part of the compiler pipeline depends on our selected optimization.
% In contrast, when we consider an optimization that does not affect other optimizations. Then the only bug we can find is inside this optimization, rather than diverse optimizations on which this optimization depends. 

To construct a deoptimization, we start by selecting a compiler optimization. Although any optimization can be chosen theoretically, we adopt two selection criteria in practice. We analyze interdependencies in the optimization pipeline and choose the top-N optimizations with the most significant influence on others~\cite{alfred2007compilers}. This approach helps us to filter out less important optimizations that are irrelevant to prominent analyses in the optimization pipeline (\eg, data flow, control flow analysis, or arithmetic operations). For example, \textit{data layout} optimization~\cite{prashantha2014implementing}, which moves a rarely accessed variable out of frequently accessed data structure, is not selected according to our criterion. Because 
% the optimization rearranges fields within objects (\eg, move a rarely accessed variable out of frequently accessed data structure), and the rearrangement 
such transformations do not affect data flow or control flow of programs. The second principle we adopt is that optimizations should be common and widely applied. This ensures that transforming deoptimized programs to their original version makes the code more natural and readable, therefore, corresponding to the optimizations that developers would have performed in real
% -world. Whereas, rare optimizations may not represent those that developers are accustomed to apply in the 
software development setting.


% The rationale is that our method detects counterproductive bugs by an optimization ``source'': a large part of the compiler pipeline depends on our selected optimization.
% Conversely, focusing on an optimization that does not impact others limits the scope of bug detection to within that specific optimization, rather than encompassing a broader range of optimizations influenced by it.


% \wyc{why, and any more criteria?} \wyc{the reason is that, we can select any optimization. but optimizations relevant to data flow or control flow may not make other optimizations performed, thus unable to detect these optimizations}
% \item Break down the optimization into a bunch of tinier independent optimization permutations at a finer granularity and randomize the permutations.

% The next step is inverting our selected optimization $opt$ to build a deoptimization $deopt$. To do the inversion, we introduce a simple model of compiler optimizations. An optimization $opt$ consisting of a precondition, a transformation and a postcondition. The precondition checks whether a code fragment can be transformed, the transformation optimizes the code fragment to a new one, and the postcondition presents the pattern of a transformed code. 
% Inverting the optimization means that the postcondition becomes the precondition, \ie, checking whether a code fragment is optimized by the optimization $opt$. The transformation part of the deoptimization comes from inverting the transformation algorithm of $opt$.  \wyc{5.14-31:00: simplify the paragraph.}
After selecting an optimization \opt, the next step is to invert \opt to construct a deoptimization \deopt. To perform this inversion, we introduce a simple model of compiler optimizations. We consider an optimization \opt as consisting of a precondition, a transformation, and a postcondition. The precondition checks whether a code fragment can be transformed, the transformation optimizes the code fragment to a new form, and the postcondition specifies the properties of the transformed code.
Inverting the optimization means that the postcondition of \opt becomes the precondition of \deopt, \ie, checking whether a code fragment has been optimized by \opt. The transformation of \deopt is derived by inverting the transformation of \opt. The precondition of \opt becomes the postcondition of \deopt, specifying the result of deoptimization.
% Although the postcondition of $deopt$ is not equivalent to the precondition of $opt$, this does not compromise our method. This discrepancy is acceptable because the postcondition of $deopt$ is not needed in the subsequent steps.


% It is worth noting that inverting the transformation is non-trivial, so we over-approximately design the inversion algorithm \st the following property holds: given an $opt$ and a program $P$ without undefined behaviors, if $P$ is transformed to $P_O$ by $opt$, when we apply $deopt$ to $P_O$ (resulting in $P_O'$), then $P_O'$ can be optimized by $opt$. %  the deoptimized code can be optimized by $opt$.
% Building on this property, although the postcondition of $deopt$ is not the precondition of $opt$, it does not break down our method because we do not require the postcondition of $deopt$ in the following steps.
% Finally, we acknowledge that some complex optimizations cannot be inverted. \wyc{check and give examples. theoretically, given an opt1, we have P (no UB) to P' by opt1, then we can have opt1', translating P' to P'', such that P'' can be optimized by opt1. but we cannot do semantically equivalent invert opt1. } 
% It is important to note that inverting compiler optimization is non-trivial. Compiler optimization often involves multiple-to-one mappings, where multiple distinct programs can be optimized into the same program. Consequently, our deoptimization cannot precisely recover the original program from an optimized version. Despite this, it does not imply that we can invert optimizations without any restriction. 
% Instead, we must design the inversion algorithm in an over-approximate manner to ensure that the deoptimized program can be re-optimized by the optimization from which the deoptimization is inverted. \wyc{or  ... can be re-optimized by the same optimization.}
% Formally, we define the following property:

% \begin{definition}[Re-optimiable]
% 	\label{def:reopt}
% 	% Given an optimization $opt$ and a program $P$ without undefined behaviors, if $P$ is optimized to $P_o$ by $opt$, then when we apply $deopt$ to $P_o$ (resulting in $P_d$), the \textit{TODO} property holds when $P_d$ can be re-optimized by $opt$.
% 	%	Given a deoptimization $deopt$ inverted from $opt$ and a program $P$ without undefined behaviors, a deoptimization $deopt$ satisfies the \textit{Reoptimiable} property when we deoptimize $P$ by $deopt$ to produce $P'$, $P'$ is guaranteed to satisfy the precondition of $opt$.
% 	Given a deoptimization \deopt inverted from \opt and programs $\mathcal{P}$ without undefined behaviors,  $deopt$ satisfies the \textit{Re-optimiable} property when the following requirement holds:
% 	$$
%     \frac
%     {
%     \begin{array}{c}
%         \forall P \in \mathcal{P}, P' = deopt(P)
%     \end{array}
%     }
%     {
%     \begin{array}{c}
%         P' \text{satisfies the precondition of }\opt \\
%     \end{array}
%     }
% 	$$
% \end{definition}
% % This property reflects the scenario of counterproductive bugs, \ie, given a program $P'$, a developer may manually optimize $P'$ to $P$ by applying $opt$ to $P'$. 
% % Although the postcondition of $deopt$ is inequivalent to the precondition of $opt$, this does not undermine our method. This discrepancy is acceptable because we do not require the postcondition of $deopt$ in the subsequent steps.

% % With this property, $P'$ is guaranteed to be optimizable by $opt$ because $P'$ satisfies the precondition of $opt$.
% % The reason for introducing this properly is that our approach reflects the semantics of counterproductive. 
% % Specifically, given a program $P'$, we can say that it is possible for a developer to manually optimize $P'$ to $P$ by applying $opt$.
% % Then, when we found that $P'$ outperforms $P$, we can claim that we found a counterproductive bug. 
% % Otherwise, we cannot draw the conclusion because $P'$ might not be optimized by $opt$.

% According to this property, $P'$ is guaranteed to be optimizable by \opt because $P'$ satisfies the precondition of \opt.
% % The reason for introducing this property is to capture the semantics of counterproductive optimizations.
% The reason for introducing this property is to simulate the scenario of finding compiler defects that lead to the mishandling of developers' optimizations.
% Specifically, with this property, it is possible for a developer to manually optimize the deoptimized program $P'$ to $P$ by applying \opt.
% If we then find that $P'$ outperforms $P$, we can conclude that we have identified a mishandling defect.
% Otherwise, we cannot make this conclusion because, without this property, developers cannot optimize $P'$ to $P$ by \opt, which invalidates our approach.


% Following our deoptimization procedure, we design a list of deoptimizations, which are shown in 
Table~\ref{table:transforms} shows the list of deoptimizations we design. All the deoptimizations are inverted from optimizations selected according to our proposed criteria. Specifically, these optimizations modify the instructions and structure of the original program and thus impact various compiler optimization components, including control flow, memory, and arithmetic optimizations. In addition, they are also common, natural, representing the set of optimizations that developers often apply to reduce code size or improve runtime performance in real-world programming.

% \wyc{todo: can remove}
% We take \textit{InstExpand} as an example. The name \textit{InstExpand} is derived from \textit{InstCombine}, an arithmetic optimization designed to reduce the number of instructions, memory accesses, or execution time required for arithmetic computations while preserving the program's correctness. 
% The optimization transforms \myinline{a && b} to \myinline{!(!a || !b)}, where \myinline{a} and \myinline{b} are two variables. The precondition, transformation, and postcondition of this optimization are \myinline{a && b}, \myinline{a && b} $\rightarrow$ \myinline{!(!a || !b)}, and \myinline{!(!a || !b)}, respectively. According to the inversion method, the precondition of the deoptimization is \myinline{!(!a || !b)}, and the transformation is inverted from \myinline{a && b} $\rightarrow$ \myinline{!(!a || !b)} to \myinline{!(!a || !b)} $\rightarrow$ \myinline{a && b}.

% As arithmetic optimizations consist of various optimizations, we show an optimization that transforms \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} to  \myinline{A | B}, where \myinline{A} and \myinline{B} are two variables. 
% The precondition, transformation, and postcondition of the optimization are  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)},  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} $\rightarrow$   \myinline{A | B}, and \myinline{A | B}, respectively. According to our inversion method, we invert the optimization from \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} $\rightarrow$   \myinline{A | B} to \myinline{A | B} $\rightarrow$  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)}, resulting a new deoptimization.  
% After selecting the optimization, we invert the optimization procedure from \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} $\rightarrow$   \myinline{A | B} to \myinline{A | B} $\rightarrow$  \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)}, resulting a new deoptimization.  \wyc{explain it by the previous paragraph.}
% \ke{what optimizations do you choose and do not choose why? Cite dragon book, 
% then go to specific examples data-flow, control-flow} resolved



% To illustrate our method to design transformations. We take \textit{InstCombine} as an example, an arithmetic optimization and peephole optimization pass in LLVM, which combines costly instructions into cheaper ones. \\

% \textbf{\textit{Selection.}}\, In the first step, we select \textit{InstCombine} optimization. 
% \textit{InstCombine} is a common optimization in the LLVM optimization pipeline consisting of large collections of independent, invertible, and simple semantic-preserving sub-permutations. There are other choices, but it is worth noting that in principle we don't favor heavy and costly optimizations like function-inlining and global-number-valuing here. These heavy optimizations are always restricted to perform once due to incrementing compile-time. For real-world testing purposes, we should not involve their variants again in mutation. Also, the transformations that have no impact on dataflow or control flow are not considered, such as renaming variables.
% \\
% \textbf{\textit{Break down.}}\, In this step, we extract independent simple sub-permutations from \textit{InstCombine} and surround them with \myinline{if} statements with indeterministic conditions like \myinline{(rand() \% 2)}, ensuring that the permutations are executed independently and randomly.\\
% \textbf{\textit{Remove checks.}}\,
% In this step, we eliminate all profitability heuristic constraints such as folding expressions only if one of the instructions is not used elsewhere. This allows us to focus on semantic constraints, enabling us to freely perform any permutation. \wyc{unclear}
% \\
% \textbf{\textit{Invert.}}\, In addition to transformations that simplify programs, we also aim to incorporate transformations that introduce complexity. While the permutations in \textit{InstCombine} match costly instructions pattern and replace it with cheaper alternatives, such as \myinline{A | B} $\rightarrow$ \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)}, we can also reverse the process by applying corresponding inverted permutations like \myinline{\textasciitilde(\textasciitilde A | \textasciitilde B)} $\rightarrow$ \myinline{A | B}. This step enhances the diversity of transformations and equivalent programs.
% \\
% In addition to the transformations derived from peephole optimization \textit{InstCombine}, we also design and randomize a list of semantic-preserving
% transformations (as shown in Table \ref{table:transforms}). These transformations modify the instructions and structure of the seed program and thus impact various compiler optimization components, including control flow, memory, and arithmetic optimizations.

\begin{table*}
	\caption{A list of deoptimizations.}
	\centering
	\begin{tabular}{ | c | c | c | }
		\hline
		Name                       & Description                                           & Example                   \\
		\hline
		\textit{InstExpand}        & Make instructions more complex                        &

		\begin{minipage}[m]{0.5\textwidth}
			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/instexpand.c}
		\end{minipage}
		\\
		\hline
		\textit{CFGExpand}         & Make control-flow more complex                        &
		\begin{minipage}[m]{0.5\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/cfgexpand.c}

		\end{minipage}
		\\
		\hline
		\textit{Reassociation} & Reassociate expressions randomly                      &
		\begin{minipage}[m]{0.5\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/reassociate.c}

		\end{minipage}
		\\
		\hline
  %SIMD
		\textit{Scalarizing}  & \tabincell{c}{Scalarize the SIMD (Single Instruction/\\Multiple Data)  operations} & \begin{minipage}[m]{0.5\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/scalarize.c}

		\end{minipage}
		\\
		\hline
		\textit{Dehoisting}    & Put loop-invariants into loops                        & \begin{minipage}[m]{0.5\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/loopsink.c}

		\end{minipage}
		\\
		\hline
		% \textit{RandomSink}        & \tabincell{c}{Randomly sink instructions                                          \\to different basic blocks} &

		% \begin{minipage}[m]{0.55\textwidth}

		% 	\lstset{style=mystyle, numbers = none, xleftmargin=2em,frame=none}
		% 	\lstinputlisting[]{./code/mutation/sink.c}

		% \end{minipage}
		% \\
		% \hline
		% \textit{RandomMem2Reg}     & Promote stack to register                            &
		% \begin{minipage}[m]{0.55\textwidth}

		% 	\lstset{style=mystyle, numbers = left, xleftmargin=2em,frame=none}
		% 	\lstinputlisting[]{./code/mutation/mem2reg.c}

		% \end{minipage}
		% \\
		% \hline
		\textit{Reg2Mem}     & Demote register to stack                              &
		\begin{minipage}[m]{0.5\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/reg2mem.c}
			% \hline
		\end{minipage}
		\\
		\hline
		\textit{DeadCodeInsertion}    & Randomly insert dead code                             &
		\begin{minipage}[m]{0.5\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/dead.c}

		\end{minipage}
		\\
		\hline
          \begin{tabular}{@{}c@{}}\textit{DeadStore-} \\ \textit{Manipulation}\end{tabular} & Insert dead store and move stores around                         &
		\begin{minipage}[m]{0.5\textwidth}

			\lstset{style=mystyle, numbers = none, xleftmargin=0.5em,frame=none}
			\lstinputlisting[]{./code/mutation/clobber.c}

		\end{minipage}
		\\
		\hline
	\end{tabular}
	\label{table:transforms}
\end{table*}

\subsubsection{Applying Deoptimizations}
% The diversity of test cases is critical to most testing approaches~\cite{hemmati2013achieving}.
% In order to enhance the diversity of our deoptimized programs, we choose random testing~\cite{hamlet1994random} since it has been proven to be effective in various testing tasks~\cite{huang2019survey}.
After constructing deoptimizations, the next step is using them to generate new programs. Concerning the diversity of the generated programs, we balance the frequency of the application of each deoptimization. This ensures every single deoptimization has contributed to the generation of some deoptimized programs.
 % second, we cap the total number of deoptimizations applied to the original program at no more than three. Applying deoptimizations too many times could result in overly artificial code, for which compilers are unlikely to generate more efficient code than they do for original programs. Because, ultimately, compilers are not designed to optimize fringe programs that do not resemble those that developers write in the real-world.

Clearly, \pd{} produced by our deoptimization procedure is a less efficient version of \po{} according to Definition~\ref{def:le} because \po{} can be derived by applying standard compiler optimizations to \pd{}. This means that the key premise of our work --- \po is more efficient than \pd{} --- holds true. 
% \gfjc{If a compiler produces?}\ke{may check English grammar?}
Should a compiler produce more optimized code for \pd than for \po, it would suggest a deficiency in the compiler.





% We choose to randomly apply deoptimization 
% % since this strategy has been proven to be effective in various testing tasks~\cite{huang2019survey, humbatova2021deepcrime}
% Technically, we first randomly select a set of deoptimizations $deopt_i$ from Table~\ref{table:transforms}.
% Then, we randomly order these deoptimizations, forming a deoptimization sequence $(deopt_{n})_{n\in\mathbb{N}}$.
% This sequence transforms the original program $P$ into a new program $P'$. Even though $P'$ seems completely different from $P$, it maintains the same functionalities and semantics.


% \subsection{Compiler Optimization}
% \wyc{To Discuss: should we add compiler optimization discussion? i.e., Therefore, the seed program $P$ is optimized to $P_O$ at an optimization level (\eg, \textit{O3}), while the mutated program $P'$ is optimized to $P'_O$ at the same or lower optimization level (\eg, \textit{O3} or \textit{O2}). }

% In this component, we optimize the input program $P$ and the deoptimized program $P'$ respectively. 
% The core component of the compiler under tested in this article is the optimization module, which transforms one program into another more efficient program and preserves the semantics. 
% We expect the tested compiler to generate optimized programs with comparable performance after compiling equivalent programs. 
% Therefore, the seed program $P$ is optimized to $P_O$ at the \textit{O3} optimization level, while the mutated program $P'$ is optimized to $P'_O$ at the same \textit{O3} optimization level. In this way, each optimized program serves as a mirror for the other.


\subsection{Performance Checking}\label{subsec:per}
% \subsection{Compare}
% \wyc{TODO: check open source good performance checking tool.}
% \wyc{compile the whole program, fuzzing, measure function level performance.}

In this subsection, we compare the performance of \pdc, the compiled code for the deoptimized program, with \poc, the compiled code for the original program. To precisely measure the performance of the generated machine code, there are two potential approaches to consider. First, we can dynamically execute/fuzz the generated code, and measure its performance through straightforward metrics such as execution time or through more sophisticated techniques like profiling. However, both approaches have limitations. Accurately measuring execution time is exceedingly challenging, if not impossible, due to factors such as non-determinism in process scheduling~\cite{barrett2017virtual}. Additionally, given that our deoptimizations are implemented at the instruction or basic block level, conventional profilers may yield imprecise results~\cite{chen2010taming}.



\begin{algorithm}[t]
	% \footnotesize
	% \captionsetup{font=scriptsize}
	\algnewcommand\Ins{$I$\xspace}
	\algnewcommand\OP{\poc}
	\algnewcommand\Prog{$P$\xspace}
	\algnewcommand\DP{\pdc}
	\algnewcommand\TI{$totalIns$\xspace}
	\algnewcommand\TC{$cost$\xspace}
	\algnewcommand\DTI{$totalIns'$\xspace}
	\algnewcommand\DTC{$cost'$\xspace}
	\algnewcommand\SQ{$deoptSeq$\xspace}
	\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}

	\caption{Estimate Performance.}
	\label{alg:ep}
	\begin{algorithmic}[1]
		\Procedure{EstimatePerformance}{\Prog}

		\State \TI $\gets$ \textit{CountInstructions}\! ({\Prog}) \label{line:ep:ci}
		% \LineComment{\hspace*{0.82em} \(\triangleright\)   traversing all subsets of `statements' in ascending \hspace*{1.6em} order of size; `-1' excludes the entire set.}
		% \LineComment{\ \ \ \ \hspace{\algorithmicindent}    cardinality; `-1' excludes the entire set.}
		\State \TC $\gets$ 0 \label{line:ep:tc0}
		\Foreach{\Ins $\in$ \Prog} \Comment{For each instruction in the program.}
		% \LineComment{\ \ \ \ \hspace{\algorithmicindent} // Ignore corner cases with which }
		% \If{\textit{filter}\! ({\Ins})}  \label{line:verifysimp}	
		\State \TC $\gets$ \TC + \textit{CostModel}\! ({\Ins})
		% \EndIf						
		\EndForeach
		\State  \Return{\TI, \TC} \label{line:ep:mpret}

		\EndProcedure
	\end{algorithmic}
\end{algorithm}

% Consequently, dynamically measuring performance is inappropriate for our approach.
% Such situations are challenging for program profiling techniques to collect the execution time or trace the number of executed instructions~\cite{zuo2021jportal}. 
% To address these challenges, we leverage static analysis and design three static performance checkers. 

Given the limitations of dynamic methods, we turn to static techniques to estimate the performance of compiled code, in particular,
%  The \textit{EstimatePerformance} function in Algorithm~\ref{alg:ep} outlines our performance estimation method.
% At a high level, 
we employ two well-known, widely applied metrics ---  the total number of instructions
% (line~\ref{line:ep:ci}) 
and the total cost of instructions 
% (lines~\ref{line:ep:tc0} to~\ref{line:ep:mpret}) 
--- for performance estimation~\cite{hashimoto2016detecting, haslbeck2022few}.
% These metrics are commonly used to approximate the performance of compiled code due to their efficiency and precision~\cite{hashimoto2016detecting, haslbeck2022few}. 
The cost associated with each instruction is determined using  LLVM's cost model~\cite{llvmcostmodel}. 
Algorithm~\ref{alg:ep} outlines this performance estimation method. It should be noted that these two metrics, while useful, may not always be precise. Below, we discuss two major factors contributing to the potential imprecision:
\begin{enumerate}[leftmargin=*]
	\item \textit{Inconsistent inlining.} It is possible that some functions in \poc{} are inlined but not in \pdc{}. 
	% However, it is challenging to measure the performance of \poc and \pdc{} without knowing how the functions are called.
	This inconsistency makes it challenging to estimate the performance of \poc{} and \pdc{} without understanding how the functions are invoked.
	      % Meanwhile, compiler developers would not modify the inlining strategies for a single case. For these reasons, we choose to ignore function-inlining in this work. \wyc{todo}
    Therefore, we ignore test cases where function-inlining occurs.
	\item \textit{Inconsistent branches.} Similar to inlining, it is challenging to statically identify the most efficient control flow layouts of programs, because it depends on the hot regions of the program at runtime. For example, an \myinline{if} statement in \poc{} is
        \begin{lstlisting}[style=mystyle, basicstyle=\small\ttfamily\bfseries, numbers = none, xleftmargin=-4em,frame=none,framexleftmargin=1.5em]
        if(cond1 || cond2) foo();
        else ...;\end{lstlisting}
     % \myinline{if(cond1 || cond2)} \myinline{foo();} 
     while the counterpart in \pdc{} is 
     \begin{lstlisting}[style=mystyle, basicstyle=\small\ttfamily\bfseries, numbers = none, xleftmargin=-4em,frame=none,framexleftmargin=1.5em]
        if(likely(cond1)) foo(); 
        else if (cond2) foo(); 
        else ...;\end{lstlisting}
     % \myinline{if(likely(cond1)) foo(); else if} \myinline{(cond2) foo();}.
     where the function \myinline{likely()}, which was introduced in C++20, indicates that the associated condition is expected to be true. This information can be used to optimize the generated machine code for better performance, such as arranging branches or prefetching to minimize pipeline stalls on modern CPUs. In this scenario, if \myinline{cond1} is in fact \myinline{true} most of the time, then the performance of \pdc{} is likely surpass the performance of \poc{}. However, if \myinline{cond1} happens to be false more frequently than anticipated, then \pdc{} could underperform compared to \poc{} due to the significant overhead caused by flushing and restarting the instruction pipeline. So, all things considered, 
     % Depending on the probability of \myinline{cond1} being \myinline{true}, \poc{} can either be more or less efficient than \pdc{}. 
     we do not count the difference between \poc{} and \pdc{} in the number and conditions of branches, in the cases where that is the only difference between \poc{} and \pdc{}, the whole test case is ignored.
 % \\Therefore, we ignore the performance difference between \poc{} and \pdc{} if they only differ in the branch conditions and the number of branches. 
		%   \wyc{chy's comment. \myinline{if (a||b) ; if (likely(a)) ...; else if (b) ...;}}
\end{enumerate}

% As we discussed in the two cases, we filter out such special cases where our performance checkers may not work precisely.
% After estimating the performance of \poc{} and \pdc{} (lines~\ref{line:cc:mp1} and~\ref{line:cc:mp2}), and our estimation is not affected by the inconsistent inlining or branches described above (line~\ref{line:cc:filterstart}), the algorithm issues a potential defect when both metrics indicate that the deoptimized program \pdc{} outperforms \poc{} (lines~\ref{line:verifysimp} to~\ref{line:cc:ccpend}). To help us manually validate these defects, we incorporate test case reduction methods (line~\ref{line:cc:report}).
% If our estimation is not affected by the inconsistent inlining or branches described above, the algorithm issues a potential defect when both metrics indicate that the deoptimized program \pdc{} outperforms \poc{}.  
% \wyc{updated: removed line numbers and test case reduction.}
% \ke{Yu, why is the overall algorithm introduced here while test case reduction, which is part of the algorithm, is not even introduced...Should make the estimation algorithm on its own and new algorithm for the entire workflow at the end of Sec 3}


% We manually validate potential defects and report valid ones to developers. 
% \ke{Yu, sounds strange here...we don't even care getting the ground-truth first? As long as the static performance estimation algorithm says there is a defect, we just report?....}\wyc{updated}





% \subsubsection{Performance Measurement}
% \wyc{overall todo: merge the following three metric into one algorithm when we do not have contributions.}

% We detect the counterproductive bugs by checking whether $P_O'$ outperforms $P_O$, so precisely measuring the performance of a program is critical for our approach.
% However, comparing the performance between programs is non-trivial, especially when deoptimized code segments cannot be executed, or worse yet, the program itself is not executable. 
% Such situations are challenging for dynamic profiling techniques to collect the execution time or trace the number of executed instructions~\cite{xxx}. 
% To address these challenges, we leverage static analysis and design three static performance checkers. 
% \wyc{we should discuss the limitation of other methods, including static performance measurement methods. Then, we explain why we use/not use these methods, and finally present our method.} 
% We consider the inconsistency between $P_O$ and $P_O'$ a missed optimization opportunity only if all the following checkers indicate that one program outperforms the other: 

\begin{algorithm}[t]
	% \footnotesize
	% \captionsetup{font=scriptsize}
	\algnewcommand\Ins{$I$\xspace}
	\algnewcommand\OP{\poc}
	\algnewcommand\Prog{$P$\xspace}
	\algnewcommand\DP{\pdc}
	\algnewcommand\TI{$totalIns$\xspace}
	\algnewcommand\TC{$cost$\xspace}
	\algnewcommand\DTI{$totalIns'$\xspace}
	\algnewcommand\DTC{$cost'$\xspace}
	\algnewcommand\SQ{$deopt$\xspace}
	\algnewcommand\CT{$counter$\xspace} 
	\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}

	\caption{Finding compiler defects.}
	\label{alg:cc}
	\begin{algorithmic}[1]
 		\LineComment{\(\triangleright\) \CT represents the frequency of the application of every deoptimization to other programs so far.
         % \gfjc{TODO explain \CT, why it is parameter and return value, }
        }
		\Procedure{FindDefects}{\po, \CT}
        \State \pd $\gets$ \po{}\label{line:cc:destart} 
        \For{$i = 0$ \textbf{to} $k$}
            \State \SQ $\gets$ \textit{selectDeoptimization}(\pd, \CT) \label{line:cc:sd}
	         \State \pd $\gets$ \textit{deoptimize}\! ({\pd, \SQ}) \label{line:cc:de}
             \State  \CT $\gets$ \textit{update}\! ({\CT, \SQ}) \label{line:cc:update}
        \EndFor\label{line:cc:deend}
        \State \OP $\gets$ \textit{compile}\! ({\po}),\, \DP $\gets$ \textit{compile}\! ({\pd})  \label{line:cc:cp}
		\State \TI, \TC $\gets$ \Call{EstimatePerformance}{\OP} \label{line:cc:mp1}
		\State \DTI, \DTC $\gets$ \Call{EstimatePerformance}{\DP}  \label{line:cc:mp2}
		\If{\textit{ImprecisionCheck}\! ({\OP, \DP})}  \Comment{Ignore special cases where the performance measurement is likely to be imprecise.}  \label{line:cc:filterstart}
		\If{\TI $>$ \DTI \textbf{and} \TC $>$ \DTC}  \label{line:verifysimp}
		\State  $R_o$ $\gets$ \textit{reduce}\! ({\po, \SQ})
        \label{line:cc:reduce}
		\State  \Return{\po, $R_o$, \CT}
		\EndIf \label{line:cc:ccpend}
		\EndIf \label{line:cc:filterend}
		% \State  \Return{False}
		\EndProcedure

		% \item[]

		% \Function{EstimatePerformance}{\Prog}

		% \State \TI $\gets$ \textit{CountInstructions}\! ({\Prog}) \label{line:cc:ci}
		% \LineComment{\hspace*{0.82em} \(\triangleright\)   traversing all subsets of `statements' in ascending \hspace*{1.6em} order of size; `-1' excludes the entire set.}
		% % \LineComment{\ \ \ \ \hspace{\algorithmicindent}    cardinality; `-1' excludes the entire set.}
		% \State \TC $\gets$ 0 \label{line:cc:tc0}
		% \Foreach{\Ins $\in$ \Prog} \Comment{For each instruction in the program.}
		% % \LineComment{\ \ \ \ \hspace{\algorithmicindent} // Ignore corner cases with which }
		% % \If{\textit{filter}\! ({\Ins})}  \label{line:verifysimp}	
		% \State \TC $\gets$ \TC + \textit{CostModel}\! ({\Ins})
		% % \EndIf						
		% \EndForeach
		% \State  \Return{\TI, \TC} \label{line:cc:mpret}

		% \EndFunction
	\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[t]
% 	% \footnotesize
% 	% \captionsetup{font=scriptsize}
% 	\algnewcommand\Ins{$I$\xspace}
% 	\algnewcommand\OP{\poc}
% 	\algnewcommand\Prog{$P$\xspace}
% 	\algnewcommand\DP{\pdc}
% 	\algnewcommand\TI{$totalIns$\xspace}
% 	\algnewcommand\TC{$cost$\xspace}
% 	\algnewcommand\DTI{$totalIns'$\xspace}
% 	\algnewcommand\DTC{$cost'$\xspace}
% 	\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}

% 	\caption{Finding compiler defects.\ke{Yu, for overall algorithm please 1. change the input parameter to \po{}, 2. add a statement to deoptimize \po{} to \pd{}, 3, another statement to compile \po{} to \poc{}, and \pd{} to \pdc{}, 4. add a return statement to return the final, reduced program from \po{}.}}
% 	\label{alg:cc}
% 	\begin{algorithmic}[1]
% 		\Procedure{FindDefects}{\OP, \DP}
% 		\State \TI, \TC $\gets$ \Call{EstimatePerformance}{\OP} \label{line:cc:mp1}
% 		\State \DTI, \DTC $\gets$ \Call{EstimatePerformance}{\DP}  \label{line:cc:mp2}
% 		\If{\textit{ImprecisionCheck}\! ({\OP, \DP})}  \Comment{Ignore special cases where the performance measurement is likely to be imprecise.}  \label{line:cc:filterstart}
% 		\If{\TI $>$ \DTI \textbf{and} \TC $>$ \DTC}  \label{line:verifysimp}
% 		\State  \textit{Reducing}\! ({\OP}) \label{line:cc:report}
% 		% \State  \Return{True}
% 		\EndIf \label{line:cc:ccpend}
% 		\EndIf \label{line:cc:filterend}
% 		% \State  \Return{False}
% 		\EndProcedure

% 		\item[]

% 		\Function{EstimatePerformance}{\Prog}

% 		\State \TI $\gets$ \textit{CountInstructions}\! ({\Prog}) \label{line:cc:ci}
% 		% \LineComment{\hspace*{0.82em} \(\triangleright\)   traversing all subsets of `statements' in ascending \hspace*{1.6em} order of size; `-1' excludes the entire set.}
% 		% \LineComment{\ \ \ \ \hspace{\algorithmicindent}    cardinality; `-1' excludes the entire set.}
% 		\State \TC $\gets$ 0 \label{line:cc:tc0}
% 		\Foreach{\Ins $\in$ \Prog} \Comment{For each instruction in the program.}
% 		% \LineComment{\ \ \ \ \hspace{\algorithmicindent} // Ignore corner cases with which }
% 		% \If{\textit{filter}\! ({\Ins})}  \label{line:verifysimp}	
% 		\State \TC $\gets$ \TC + \textit{CostModel}\! ({\Ins})
% 		% \EndIf						
% 		\EndForeach
% 		\State  \Return{\TI, \TC} \label{line:cc:mpret}

% 		\EndFunction
% 	\end{algorithmic}
% \end{algorithm}


% \subsubsection{Performance Measurement}
% \wyc{overall todo: merge the following three metric into one algorithm when we do not have contributions.}

% We detect the counterproductive bugs by checking whether $P_O'$ outperforms $P_O$, so precisely measuring the performance of a program is critical for our approach.
% However, comparing the performance between programs is non-trivial, especially when deoptimized code segments cannot be executed, or worse yet, the program itself is not executable. 
% Such situations are challenging for dynamic profiling techniques to collect the execution time or trace the number of executed instructions~\cite{xxx}. 
% To address these challenges, we leverage static analysis and design three static performance checkers. 
% \wyc{we should discuss the limitation of other methods, including static performance measurement methods. Then, we explain why we use/not use these methods, and finally present our method.} 
% We consider the inconsistency between $P_O$ and $P_O'$ a missed optimization opportunity only if all the following checkers indicate that one program outperforms the other: 




% \vspace*{3pt}
% \noindent
% \textbf{\textit{Counting the instructions.}}\,
% This checker counts the number of instructions in the optimized code (\ie, $P_O$ and $P_O'$).
% \wyc{explain why we choose it: combine three, to reduce FP. reason 1: other work also uses it.} 
% Though optimizations like loop unrolling produce larger programs, in most cases, the instruction count reduction indicates a performance improvement. 
%This checker shows interestingness only if $P_O$ and $P_O'$ differ in the instruction count. \wyc{can we address "loop unrolling produce larger programs"? \eg, use this checker when we know loop unrolling is not performed.}


% \vspace*{3pt}
% \noindent
% \textbf{\textit{Estimating cost by static profiling.}}\, 
% In most cases, the tested programs are indeterministic and not executable. We cannot simply use dynamic profiling techniques to calculate the execution time or the number of executed instructions. Instead, we design a static analysis method to estimate the cost of given programs. 
% \citet{static-profile} proposed a static \textit{program-based} branch probability predictor. LLVM implemented a similar predictor in \textit{Branch Probability Info} and \textit{Block Frequency Analysis}. With the tools above, the performance checker estimates the cost of a given program by following the steps below:
% \wyc{check: discuss with hongyu.}
% We follow a static \textit{program-based} branch probability predictor proposed by \citet{static-profile} to estimate the cost of a program.
% Particularly, we estimate the cost following the steps below:
% \begin{enumerate}
% 	\item For every basic block $b_i$, we estimate the execution frequency $f(b_i)$ of each basic block by the static predictor.
% 	\item Calculate the cost $c(b_i)$ of basic block $b_i$ by adding up the cost of all instructions in $b_i$. In this step, we model the cost of every single instruction with \textit{Cost Model} of \textit{LLVM}. \wyc{to discuss, what is cost model}
% 	\item Sum up the cost of all basic blocks: $\sum_{i}{f(b_i) \cdot c(b_i)}$ as the estimated total cost.
% \end{enumerate}
% The lower the cost is, the faster the program possibly is. 
% This checker shows interestingness only if $P_O$ and $P_O'$ differ in the estimated cost.



% \vspace*{3pt}
% \noindent
% \textbf{\textit{Uninterested set.}}\,
% \wyc{maybe become a part of the algorithm filtering.}
% The performance checkers above cannot cover all cases precisely in practice. We extract some common static characteristics found in uninterested results:
% \begin{enumerate}
% 	\item \textit{Inconsistent inlining.} In some cases, some functions in one program are inlined, while those of the other are not inlined. However, it's hard to measure the profitability of function-inlining without knowing how the functions are called externally. Meanwhile, compiler developers would not modify the inlining heuristics for a single case. For these reasons, we don't test function-inlining in this work.
% 	\item \textit{Inconsistent only with branches.} Similar to inlining, it's hard to decide which layout of the control-flow graph of programs is better at compile time, which depends on the hot regions of the program at runtime. We are not interested if the difference between $P_O$ and $P_O'$ is only the number of branch instructions. \wyc{one branch less instructions, and the other has more.}
% \end{enumerate}
% In our testing, we filter out all irrelevant results that exhibit these characteristics to ensure that the outcome does not contain a significant number of false positives.






% \begin{algorithm}[t]
% 	% \footnotesize
% 	% \captionsetup{font=scriptsize}
% 	\algnewcommand\Ins{$I$\xspace}
% 	\algnewcommand\OP{$P_O$\xspace}
% 	\algnewcommand\RP{$R$\xspace}
% 	\algnewcommand\DRP{$R'$\xspace}
% 	\algnewcommand\Prog{$P$\xspace}
% 	\algnewcommand\DP{$P_O'$\xspace}
% 	\algnewcommand\TI{$totalIns$\xspace}
% 	\algnewcommand\TC{$cost$\xspace}
% 	\algnewcommand\DTI{$totalIns'$\xspace}
% 	\algnewcommand\DTC{$cost'$\xspace}
% 	\algnewcommand\DS{$DeoptSeq$\xspace}
% 	\algnewcommand\OL{$OptLevel$\xspace}
% 	\algnewcommand\RO{$R_O$\xspace}
% 	\algnewcommand\DRO{$R_O'$\xspace}
% 	\algblockdefx[Foreach]{Foreach}{EndForeach}[1]{\textbf{foreach} #1 \textbf{do}}{\textbf{end foreach}}

% 	\caption{Test Case Reduction. }
% 	\label{alg:tcr}
% 	\begin{algorithmic}[1]
% 		\Procedure{TestCaseReduction}{\OP, \DS, \OL}
% 		\State $P$ $\gets$ \OP
% 		\Do
% 			% \If{\textit{Filter}\! (\RP)}  
% 			% \State  \textit{ReportCounterproductive}\! ({\OP})
% 			% \EndIf 
% 			\Do
% 				\State \RP $\gets$ \textit{Reduce}\! ({$P$})
% 			\doWhile{\textit{Filter}\! (\RP) \textbf{or} \RP is $\emptyset$} 
% 			% \State \DRP $\gets$ \textit{ApplyDeoptimization}\! ({\OP, \DS}) 
% 			% \State \RO $\gets$ \textit{Compile}\! ({\RP, \OL}),  \DRO $\gets$ \textit{Compile}\! ({\DRP, \OL}) 
% 			% \State \TI, \TC $\gets$ \Call{CheckCounterproductive}{\RO, \DRO} 
% 	  	\doWhile{\textit{counterproductiveFound}\! (\RP)} 
% 		\State \Return{\RP}
% 		\EndProcedure

% 	\end{algorithmic}
% \end{algorithm}

% As bug-triggering input programs tend to be too large and complex for human developers to understand, an automated test-case reduction tool is an essential component of a compiler testing setup~\cite{lecoeur2023program}. 
\subsection{Test Case Reduction}\label{subsec:red}
When \pdc{} is estimated to outperform \poc{}, we need to reduce \po{} for human consumption, considering that \po{} used in this work is a large program consisting of hundreds of lines of code.
Our reduction procedure ensures the following two conditions: (1) the reduced program remains well-defined; (2) the reduced program continues to trigger the compiler defect resulting in the superior performance of \pdc{} to \poc{}.

% \begin{algorithm}[H]
% \caption{Counting from 0 to 10}
% % \SetAlgoLined
% \For{$i \leftarrow 0$ \KwTo $10$}{
%     \tcp{}
%     \textbf{print} $i$\;
% }
% \end{algorithm}


We utilize the automatic test case reducer~\cite{regehr2012test} 
to reduce a program $P$. Basically, for a reduced program $R$, we repeat the previous steps, \ie, transforming $R$ to $R'$ with the identical deoptimization sequence that transforms \po{} to \pd{}, compiling $R$ to $R_c$, and $R'$ to $R_c'$ by the same optimization level, and checking whether $R_c'$ still outperforms $R_c$. However, we face two potential issues:
\begin{enumerate}[leftmargin=*]
	\item We cannot guarantee that the same compiler defect can still be triggered by the reduced program~\cite{reduce-vary}. Unlike crash or mis-compilation bugs, defects that lead to compilers mishandling developers' optimizations are more prone to this issue because our performance checkers are less precise.
	\item The superior performance estimated from $R_c'$ to $R_c$ may be due to the 
 % reduced program may contain undefined behavior. The compiled code for the Test-case reducer can yield a small program that appears to be a mishandling defect, but the issue is actually caused by 
    undefined behavior in $R$. For example, $R$ contains a division by zero (\ie, \myinline{a/0}) which causes undefined behavior. Specifically, \myinline{a/0} in $R$ might be compiled to \myinline{a + 1} in $R_c$, while \myinline{a/0} in $R'$ might be compiled to \myinline{0} in $R_c'$. Although \myinline{0} is more optimized than \myinline{a/0}, this does not mean that compilers mishandled $R$.
\end{enumerate}

To ensure that the reduced program preserves the properties of the original program, we design the following two checks. 
% In particular, any reduced program that violates either of these two checks will be rejected.
%\footnote{Rejecting a reduced program does not mean we discard it. For example, violating the first check depicts that we may find another mishandling defect. \ke{don't understand this part, sounds very adhoc and engineering}}. 
\begin{itemize}[leftmargin=*]
    \item \textbf{\textit{Consistent contrast.}}\,
    We analyze the characteristics of $R_c$ and $R_c'$, and require the contrast of their characteristics to be consistent with the contrast between the characteristics of \poc and \pdc. Technically, we define the contrast between the characteristics of two machine code as the variance in the number of identical types of instructions. That is, the difference between the number of identical types of instructions in $R_c$ and $R_c'$ must align with that between \poc and \pdc. For instance, if the number of \myinline{add} instructions in \pdc is fewer than in \poc, then the number of \myinline{add} instructions in $R_c'$ must also be fewer than in $R_c$.
    \item \textbf{\textit{Undefined behavior checking.}}\, Since the reducer does not guarantee the absence of undefined behavior in the reduced program, we design undefined behavior checks following LLVM's documentation~\cite{llvmpoison, llvmub} (\eg, preventing load from \myinline{null} pointer, imposing checks on the range of values to guard against overflow/underflow).
 
 
 
 % \ke{Yu, Give some examples?}, \eg undefined behaviors like load from a null pointer, Signed integer overflow. 
 %    \wyc{Below we give two undefined behavior examples:}
	% \begin{lstlisting}[style=mystyle, basicstyle=\small\ttfamily\bfseries, numbers = none, xleftmargin=-4em,frame=none,framexleftmargin=1.5em]
 %      int fun(int a, int b, int* p) {
 %        int ret;
 %        if(p != NULL) return use(p);
 %        ret = *p; // Load from null pointer
 %        if(a > 123 && b >= 0x7FFFFFFE)
 %          return a + b; // Signed integer overflow
 %        else return ret;
 %      }\end{lstlisting}
\end{itemize}

\subsection{Overall Algorithm}
% \wyc{updated the algorithm, but this section seems similar to section 2.2.}

Algorithm~\ref{alg:cc} depicts our overall algorithm. Given the original program \po{} and how frequent every deoptimization has been applied to other programs so far (recorded by the input parameter $counter$), we generate deoptimized programs by repeatedly applying a deoptimization to the current state of the program for a number of times $k$ (line~\ref{line:cc:destart} to~\ref{line:cc:deend}). We set $k$ to be 15. A larger value of $k$ only increases the cost of computation without improving the results.
% and the distribution of the application of every deoptimization so far (lines~\ref{line:cc:sd}). 
Then, we compile the original program \po{} and the final deoptimized program \pd{} to machine code \poc{} and \pdc{} respectively (line~\ref{line:cc:cp}).
After estimating the performance of \poc{} and \pdc{} (lines~\ref{line:cc:mp1} and~\ref{line:cc:mp2}) according to Algorithm~\ref{alg:ep}, and our estimation is unaffected by
% \gfjc{ignores?} \ke{we did ignore...}
inconsistent inlining or branches described at Section~\ref{subsec:per} (line~\ref{line:cc:filterstart}), the algorithm returns \po{}, $R_o$, and $counter$ when both metrics indicate that the deoptimized program \pdc{} outperforms \poc{} (line~\ref{line:verifysimp} to~\ref{line:cc:ccpend}). The \textit{reduce} function at line~\ref{line:cc:reduce} reduces \po{} to $R_o$ according to the procedure described in Section~\ref{subsec:red}. 
% The \textit{update} function at line~\ref{line:cc:update} records the latest distribution of the application of every optimization after $deoptSeq$ is applied to \po{}.

==> overview.tex <==



==> pre <==
% \subsection{Preliminary}
% \label{subsec:pre}

% In this section, we give a brief overview of compiler optimizations. For clarity, we use a simple compiler, \cmp, to illustrate the key concepts.

% Like any typical compiler, \cmp takes a program written in a language $\mathscr{L}$ (with semantics $\llbracket \cdot \rrbracket$) and compiles it into machine code. Since the focus of this work is on compiler optimizations, we formalize the optimization procedure in \cmp.

% \cmp relies on a set of optimization phases (or optimization passes) $\Phi$ to optimize an input program. Each optimization phase $\phi \in \Phi$ consists of a sequence of semantically-preserving program transformations $T_\phi$ (\eg, removing deadcode, replacing expressing with constants, moving loop invariants out of the loop). Here, we use the subscript to denote the optimization phase $\phi$ that $T_\phi$ belongs to. By combining the transformations from all optimization phase in \cmp, we obtain the entire set of transformations $\mathcal{T}$ that \cmp uses for optimization
% \[ \mathcal{T} = \bigcup\limits_{\forall \phi \in \Phi} \mathit{set}(T_{\phi}) \]
% where $\mathit{set}(\cdot)$ is a function that converts sequences to sets (by ignoring the order of elements and removing duplicates in an sequence). Given the set of all transformations $\mathcal{T}$, it follows that $T_{\phi} \in \mathcal{T}^{*}$ where $*$ denotes the Kleene star.
% % $T \in \mathcal{T}^*$, where $\mathcal{T}$ is the set of transformations resulted from the combination of every transformation from every optimization phase in \cmp. 

% Each transformation $t \in \mathcal{T}$ is a function $t: \mathscr{L} \rightarrow \mathscr{L}$ that receives a program $P$ as input, and generates another program $Q$ as output, assuming \cmp's optimization operates at the source code level (\ie, in language $\mathscr{L}$). When \cmp applies an optimization phase $\phi$ to an input program, essentially, it applies $T_\phi$ to the program. This means that each individual transformation $t_i$ in $T_\phi$ is successively applied to the result of the previous transformation. For example, given a program $P$ and $T_\phi=(t_1,t_2,\dots,t_n)$, the application of $T_\phi$ to $P$ is defined as $T_\phi(P) = t_n(\dots t_2(t_{1}(P)))$. Similarly, applying multiple optimization passes $\varphi=(\phi_1,\phi_2,\dots,\phi_n)$ to $P$ can be formalized into $\varphi(P) = T_{\phi_{n}}\dots(T_{\phi_{2}}(T_{\phi_{1}}(P)))$.

% We use a function $\delta:\mathscr{L} \rightarrow \mathbb{R}_{>0}$ ($\mathbb{R}_{>0}$ denotes the set of positive real numbers) to measure the efficiency of a program. Specifically, $\delta(Q) > \delta(P)$ means $Q$ is more efficient than $P$. In principle, function $\delta(\cdot)$ could depend upon code size, expected runtime, number of disk accesses, power consumption, or any other measure of resource usage. In this paper, we focus on code size, and expected/actual runtime to measure the efficiency of a program.

% % do not differentiate these implementation choices for $\delta(\cdot)$ and assume it to be a pre-defined function directly given to \cmp.

% Finally, we formalize the phase ordering problem in \cmp. Given a program $P$ to optimize, the goal is to find an ordering of optimization passes $\varphi \in \Phi^*$, such that applying $\varphi$ to $P$ results in the most efficient code. Formally, we seek an ordering $\varphi$ where no other ordering  $\varphi^\prime \in \Phi^*$ produces a more efficient program
% $\nexists \varphi^{\prime} \in \Phi^* \delta(\varphi^{\prime}(P)) > \delta(\varphi(P))$.









% \ke{revise, optimal ordering means optimal sequence of transformations (may across phases)}
% we now formalize the existing procedure of compiler optimizations. Given a program $P$, \cmp (or any typical compiler) attempts to find a sequence of transformations $T_P$,
% %$ =\{t_{P_1},t_{P_2},\cdots,t_{P_n}\}$, 
% such that applying $T_P$ to $P$
% % each transformation $t_{P_i}$ in $T_P$ in turn, denoted by $P_1=t_{P_1}(P), P_2=t_{P_2}(P_1),\cdots,Q=t_{P_n}(P_{n-1})$, 
% results in the most efficient program $Q$. That is, out of all sequences of transformations that \cmp could have applied, applying $T_P$ to $P$ generates the most efficient code, formally, $\nexists T \in \mathcal{T}^* \phi(T(P)) > \phi(T_P(P))$. In fact, such process of finding the optimal sequence $T_P$ for a program $P$ is essentially solving the classical phase ordering problem~\cite{po1,po2,po3,kulkarni2006exhaustive}.

